The Hidden cost of the Edge: A Performance Comparison of Edge and Cloud Latencies

Edge computing has emerged as a popular paradigm for running latency-sensitive applications due to its ability to offer lower network latencies to end-users. In this paper, we argue that despite its lower network latency, the resource-constrained nature of the edge can result in higher end-to-end latency, especially at higher utilizations, when compared to cloud data centers. We study this edge performance inversion problem through an analytic comparison of edge and cloud latencies and analyze conditions under which the edge can yield worse performance than the cloud. To verify our analytic results, we conduct a detailed experimental comparison of the edge and the cloud latencies using a realistic application and real cloud workloads. Both our analytical and experimental results show that even at moderate utilizations, the edge queuing delays can offset the benefits of lower network latencies, and even result in performance inversion where running in the cloud would provide superior latencies. We finally discuss practical implications of our results and provide insights into how application designers and service providers should design edge applications and systems to avoid these pitfalls.

==> 04_validation_ahmed.tex <==
\section{Experimental  Comparison}
\label{sec:eval}

Having analytically compared edge and cloud latencies from the perspective of performance inversion, we now experimentally compare the two using realistic applications and real cloud workloads.
%In the previous section, we used analytical models---based on queuing theory--- to analyze scenarios where edge performance inversion can occur. We next show experimentally that performance inversion can occur in real cloud and edge settings when running realistic applications. 
\subsection{Experimental Setup}

\noindent \textbf{Edge/Cloud deployments.} To demonstrate that edge performance inversion can occur in real world 
settings, we conduct our experiments on Amazon's EC2 cloud. The EC2 cloud platforms offers numerous choices of cloud data center 
locations which allows us to conduct experiments on cloud servers with different network latencies. 
We utilize these choice of data center locations to experiment with different edge and cloud application scenarios with different network latencies. All our experiments assume an edge round trip latency of 1ms, which represents the best case scenario for edge deployments. We do so by placing the end client (emulated using a workload generator) and the edge servers in two different availability zones (data centers) within the same EC2 availability region, yielding a very low user-to-edge network lantecy.
We use three different cloud deployments to complement our 1ms edge deployment.\\
Our first scenario assumes a \emph{nearby} cloud that is around 15ms away, yielding a small $\Delta n$ ($\Delta n < 20$). As the number of  cloud data centers has grown, it is now feasible for a cloud server to have less than 20m round trip time (RTT) latency from the user.  We place the end-client and the edge servers in the us-east-2 EC2 region (in Ohio), and the cloud servers  in the us-east-1 in Virginia, with an average Round-Trip-Time (RTT) of around 15 ms.~\footnote{We also ran similar experiments with the edge in Ireland and the Cloud in London, but omit these results since they are similar.}\\
Our second scenario assumes a cloud that is between 20 to 30 ms away, yielding a medium  $\Delta n$ ($\Delta n \sim 20$). This is an increasingly common latency seen by end-users in populated urban centers. Our experiments use two configurations. We use an  edge deployment  in Ireland, and a cloud deployment   in Frankfurt, yielding a network RTT between 20 to 24 ms.  We also use an edge deployment in us-east-2 (Ohio),and a cloud deployment in ca-central-1 (Montreal) with an RTT time between 25 to 28 ms.\\
Our third scenario assumes a cloud that is located over 50ms away, yielding a larger $\Delta n$ ($\Delta n > 50$).  Users in many parts of the world may still experience cloud RTTs that exceed 50ms. It is also common to experience higher RTT latencies when using a cellular connection.  In this case, we deploy the edge and end-clients in us-east-2 (Ohio) and the cloud in us-west-1 (North California), with an average RTT of around 50 to 60 ms.\\
Finally, we also experiment with a distant cloud application by deploying the edge  in the US  (us-east-1), and the cloud in Europe, with latencies exceeding 120 ms. Since this involves crossing trans-continental ocean links, we assume that well-designed geo-distributed applications will avoid such scenarios and omit detailed results and present brief summaries where applicable. 

All experiments assume the same configuration  for the  cloud and edge servers; we use the c5a.xlarge instance type, with 4 vCPUs, 8 GB of memory, and 10GB/s network inferences. We assume that the cloud deployment of the applications runs on  5, 10, or 20 servers in the cloud, while corresponding edge deployments use one or two servers at each site.  In the cloud case, we use HA-Proxy, a popular load-balancer to balance the load across the different cloud servers.





%To validate our models, we run experiments in a number of different AWS locations, with various choices of where we locate the edge deployment, the cloud deployment, and the workload generator---emulating the users---governing the latencies in the system. We choose to always deploy the workload generator and the edge deployment within 1 ms, a best case scenario for any edge cloud system. To do so, we use the fact that each AWS site has multiple availability zones---data centers that are located near each other within the same region. We choose to validate our models with three main scenarios:
%\begin{enumerate}
%    \item The case where $\Delta n$ is small, and the cloud is located less than 20 ms away. Today, the latency between users and cloud deployments can be less than 20 ms. For these experiments we choose to test with one configuration; the edge deployment is located in the us-east-2 region (in Ohio), and the cloud deployment is located  in the us-east-1 in North Carolina, with an average Round-Trip-Time (RTT) of around 15 ms.~\footnote{We ran similar experiments with the edge in Ireland and the Cloud in London, but do not show the results as they were redundant}
%    \item The case where $\Delta n$ is medium, and the cloud is located between 20 to 30 ms away. This is a common latency seen today between users and cloud servers. For these experiments we choose to test with two configuration; The edge deployment  located in Ireland, and the cloud deployment  located in Frankfurt, with the Round-Trip-Time (RTT) between 20 to 24 ms; The edge deployment in us-east-2 (Ohio), and the cloud deployment in ca-central-1 (Montreal) with an RTT time between 25 to 28 ms.
%    \item The case where $\Delta n$ is large, and the cloud is located over 50 ms away. This scenario is becoming less and less common in many regions in the world with more advanced Internet infrastructures. However, in some cases, e.g., in more remote areas, on bad wireless links, or when the application is deployed in a single region, these scenarios can occur. We test one configuration for this case where the edge is located in us-east-2 (Ohio) and the cloud is located in us-west-1 (North California), with an average RTT of around 50 to 60 ms.
%\end{enumerate}
%We have also tested with longer latencies, deploying the application in a US data center, and the cloud in Europe, with latencies exceeding 120 ms. However, we decided to omit these results as these would represent a less common scenario.
%
%Finally, for all our cloud and edge servers, we use the c5a.xlarge instance type, each of which having 4 vCPUs and 8 GB of memory. We assume that the application runs on either one or two servers on the edge, and runs on 5, 10, or 20 servers in the cloud. In the cloud case, we use HA-Proxy, a popular load-balancer to balance the load across the different cloud servers.

\noindent\textbf{Application Workload}  Since many type of edge applications such as mobile AR, virual analytics and IoT processing involve some form or machine learning, we choose deep neural network (DNN) inference workload for our experiments. The application is a web-based  DNN image classification service  built using  Keras, TensorFlow,  and Flask that is designed to receive image requests from an end-client and responds with the class of the image. Note that this is more compute-intensive workload than simple web applications.

We built a workload generator using Gatling, an open-source load- and performance-testing framework based on Scala. We choose Gatling for its scalability. We use a large images dataset from Kaggle. Each second, the workload generator randomly selects a set of images, based on the number of requests configuration for the experiment, and sends them to the edge application for classification. When the response is received, the workload generator logs the end-to-end response time.  The workload generator is capable of generating requests that follow a specified distribution or it can replay a request trace.

The application and our workload generator are part of a edge-cloud performance benchmarking tool that we have developed as part of this work (see Appendix \ref{sec:appendix}) and use automation tools for easy deployment and performance benchmarking on cloud and edge servers of global cloud platform providers.

\noindent\textbf{Azure Trace Workload}


%Since many of the most common applications scenarios to be deployed on the edge involve running Machine Learning (ML) workloads, we have chosen to validate our results with a DNN-based image classification workload. The chosen application is built using Keras, TensorFlow,  and Flask, to build an online image classification service which receives requests with an image and replies with a class for that image. This is a computationally heavy workload. 

%\noindent\textbf{Workload Generator.} We build a workload generator using Gatling, an open-source load- and performance-testing framework based on Scala. We choose Gatling for its scalability. We use a large images dataset from Kaggle. Each second, the workload generator randomly selects a set of images, based on the number of requests configuration for the experiment, and sends them to the edge application for classification. When the response is received, the workload generator logs the end-to-end response time. 

\noindent\textbf{Benchmarking the application.} Before we run any experiments, we benchmarked our application while running on the c5a.xlarge AWS instance type to find the maximum service rate that these instances can support. We found that at 13 req/s, the system reaches 100\% utilization and starts dropping requests or thrashing. We hence choose to use the service rate $\mu$ to be 12 req/s, the maximum practical sustainable workload by these instances. At this request rate, the average utilization is between 85 and 90\%.

\section{Experimental Results}
We now show how we validate our queuing models under different realistic conditions. Due to the lack of space, we only show our validation of some of our key results. 


\begin{figure*}
\centering
\captionsetup{justification=centering}
\begin{minipage}[t]{0.33\linewidth}
\centering
    \includegraphics[width=\linewidth]{figures/near_cloud_vs_edge_mean.pdf}
    \caption{Mean response time of edge (Ireland) and a typical cloud (Frankfurt) (Application with latencies of 1 ms to edge, and  20 to 30 ms to cloud.)}
    \label{fig:nearCloudl}
\end{minipage}
\begin{minipage}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/distant_cloud_vs_edge_mean.pdf}
    \caption{Mean response time of edge (Ohio) and distant cloud (North California) (1 ms to edge, and 50 ms to cloud)}
    \label{fig:distantCloud}
\end{minipage}
\begin{minipage}[t]{0.33\linewidth}
\centering
    \includegraphics[width=\linewidth]{figures/crossover_cpu.pdf}
    \caption{Average CPU utilization when crossover happens, the edge location is at us-east-2 (Ohio), Cloud deployments on the x-axis with RTTs of 15, 25 to 30, and 50 to 60 ms respectively.}
    \label{fig:cpu_util}
\end{minipage}
\end{figure*}

\subsection{Validating the models}
In our first set of experiments, we aim to validate Lemma~\ref{lemma:mmk}. To do so, we generate workloads with Poisson arrival rates using the workload generator. For each of the cloud configurations described above, we run multiple experiments, varying the average request arrival rate $\lambda$ between 6 and 12 req/s between experiments. We now discuss the results for each of these scenatios.

\noindent\textbf{For a typical application to cloud delay of 20 to 30 ms.} For this experiment, we run our experiments for the case when $\lambda_{edge}=\lambda_{cloud}/k$. Since $\mu$ is constant for all our experiments, and is set to 12 req/s, Lemma~\ref{lemma:mmk} reduces to Corrolary~\ref{corr:equal_balanced}. Since the RTT varies between each request, with many images split between multiple network packets, we set $\Delta n=30$, then for $k=5$, our model predicts that the inversion occurs when $\rho_{edge}=$ $\rho_{edge}=0.64$, and predicts that the inversion occurs at  $\rho_{edge}=0.54$ when $k=10$.

Figure ~\ref{fig:nearCloudl} shows the experimental results of a deployment where the user and edge deployment are deployed in Ireland with a latency of 1 ms on average, while the cloud application deployment is in Frankfurt (with RTT varying between 20 to 30 ms to the user).  We see that performance inversion occurs at $\lambda=8 req/s$, which corresponds to $\rho=8/13=0.61$ for both the configurations with 5 and 10 servers. This result shows that our model underestimates the inversion point by 4.5\% for the 5 servers case, and over-estimates the inversion point by 12\% for the 10 servers configuration. 
We note that this model error is a direct result of the discrete nature of changes in $\rho$ due to the very high computational requirements of the application, causing ``jumps'' in utilization values with the addition of even one single extra request.

We have done similar analysis for a scenario when the edge has 2 servers instead of only one. In this case, the analysis suggests that the inversion occurs at $\rho_{edge}=0.75$ for compared to a 10 server cloud, and 0.64 for a 5 servers cloud. Our model underestimates the inversion point by 6\% for the 10 server scenario, and by 18\% for the 5 servers cloud.

\noindent\textbf{For a high application to cloud delay of 50 to 60 ms.} For this experiment, the edge deployment is again within 1 ms from the user,  while the cloud deployment is in North California, with an average RTT varying between 50 to 60 ms. Using similar analysis, for an edge with 1 server, the theory predicts that when the cloud has 5 servers, inversion will happen at 81\% utilization with a cloud deployment of 5 servers, and at 78\% with 10 servers. Our experiments on AWS shows that the inversion occurs at 84\% utilization for both cloud deployments, with an error of less than 4\% for the 5 servers case, and less than 12\% for the 10 servers case.


Hence, the experiments shown in figures~\ref{fig:nearCloudl} and \ref{fig:distantCloud} clearly show that our models can predict the performance inversion point with high accuracy in most cases. These validation experiments show the strength of the developed models and that they can be used by practitioners to better understand the system performance before deploying their workloads.

\noindent\textbf{Performance Inversion for different cloud configurations.}
Figure~\ref{fig:cpu_util} shows the measured utilization at which performance inversion occurs for different cloud configurations. Clearly, as the $\Delta n$ shrinks to be around 15 ms, the inversion point occurs at the rather low utilization  of 40\% which occurs around $\lambda=6$. As the distance to the cloud increases, the performance inversion point occurs at higher utilizations. We note that the measured utilization at the cloud is slightly lower than what is measured on the edge due to the better multiplexing and queuing on the cloud. 


\subsection{Edge Tail Latency}
\begin{figure*}
\centering
\captionsetup{justification=centering}
\begin{minipage}[t]{0.45\linewidth}
\centering
\includegraphics[height=2 in]{figures/distant_cloud_vs_edge_p95.pdf}
    \caption{P95 response time of edge (Ohio) and distant cloud (North California)}
    \label{fig:p95}
\end{minipage}
\begin{minipage}[t]{0.45\linewidth}
\centering
\includegraphics[height=2 in]{figures/distant_cloud_vs_edge_violin_10.pdf}
    \caption{Response distribution of edge (Ohio) and distant cloud (North California) when normalized request rate = 10}
    \label{fig:violin_tail}
\end{minipage}
\end{figure*}

While our previous experiments validated some of our main analytical queuing models, we now turn our attention to something which our models do not capture, tail latency measurements on both the edge and cloud. We focus on the experiments we ran using a cloud deployment that is 50 to 60 ms away from the users emulated by the workload generator, and measure the $95th$ percentile response time. Figure~\ref{fig:p95} sheds light on a largely non-studies aspect of the effects of running applications on resource constrained edge clusters. Clearly, even with the very long latency to the cloud deployment, it provides superior P95 response time compared to an edge deployment, with a single server edge seeing worse P95 latency at around 50\% to 60\%  utilization. While adding one more server to the edge improves the tail latency at the edge, still, at around 80\% utilization, the cloud again provides superior performance to the 2-servers edge. 

To better understand the latency distributions and tails in both the edge and the cloud deployments, Figure~\ref{fig:violin_tail} shows violin plots for the response time distributions for various edge an cloud configurations when $\lambda=10$. Clearly, single server edge deployments exhibit a much longer tail even when both the average and median latencies are lower than the cloud. Adding one extra server to the edge improves the tail, however, if $\lambda$ increases, then the benefits of the extra server on the edge diminishes with respect to the tail.


\subsection{Statistical Multiplexing on the Edge}

\begin{figure*}
\centering
\captionsetup{justification=centering}
\begin{minipage}[t]{0.3\linewidth}
    \centering
    \includegraphics[height=1.6 in]{figures/azure_number_of_requests_per_source.pdf}
    \caption{The request rate of five serverless functions owned by the same owner extracted from the Azure publicly available serverless traces.}
    \label{fig:serverless}
\end{minipage}
\begin{minipage}[t]{0.3\linewidth}
    \centering
    \includegraphics[height=1.6 in]{figures/azure_cloud_vs_edge_mean.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{minipage}
\begin{minipage}[t]{0.3\linewidth}
    \centering
    \includegraphics[height=1.6 in]{figures/azure_boxplot.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{minipage}
\end{figure*}

Our final set of experiments compares the benefits of statistical multiplexing of the cloud to the benefits of proximity in the edge case. In this set of experiments, we use the publicly available serverless traces from Azure~\cite{}. We analyze the traces, and extract a subset of traces for five serverless functions owned by the same user. We assume that the workload for each of these functions is the load on one of our edge sites hosting the ML classification workload.

Figure~\ref{fig:serverless} shows the request arrival rate at each of these edges over a period of 20 minutes. We then build an experiment where the workload generator is situated in us-east-2 in Ohio, and each function workload is directed to a separate single-server edge, i.e., we distribute the load across five edge sites. The RTT between the users and the edge servers is on average 1 ms. We repeat the experiment with all five workloads are directed instead to a  five-server  cloud cluster located in ca-central-1 (in Montreal), while the workload generator is running in us-east-2. For the cloud experiment, the RTT time varys between 20 to 30 ms.
% RTT between us-east-2 and us-west-1: ~ 13ms
% RTT between us-east-2 and ca-central-1: ~ 25ms
% RTT between us-east-2 and us-west-1: ~ 50ms



==> practical.tex <==

\section{Practical implications}

\begin{figure*}
\centerline{
 \subfigure[The $\Delta T$ bound when the remote cloud is moderately loaded with average utilization of 0.6.] 
{\label{fig:ccdl}
\includegraphics[width=3.5 in, height=2 in]{figures/DelayBound_rhoc06.pdf}}
  \subfigure[The $\Delta T$ bound when the remote cloud is heavily loaded with average utilization of 0.99.] 
{\label{fig:ccdh}
\includegraphics[width=3.5 in, height=2 in]{figures/DelayBound_rhoc099.pdf}}
}
 \caption{As the edge becomes more loaded, the queuing effects increase significantly.}
\label{fig:Dbound}
 \end{figure*}
 
Our results have many practical implications on how edge computing systems should be designed. They clearly indicate many trade-offs when choosing where to offload computations.  A factor that is very important in these decisions is the system utilization at the edge servers. We now use numbers from real systems to shed light on how these trade-offs would play in real systems

\subsection{The delay bound} \label{sec:impD}
Using Equation~\ref{eq:Tau_delta}, figures~\ref{fig:ccdl} and \ref{fig:ccdh} show the maximum bound on $\Delta T$, the RTT delay difference between offloading to a remote large-scale cloud versus to a local edge cloud, as a function of the edge utilization and the size of the remote cloud when the remote cloud is moderately and highly loaded respectively. When the remote cloud is moderately loaded at 60\% utilization, the bound depends only on the edge utilization. On the other hand, when the remote cloud is highly loaded at 99\% utilization, the size of the remote cloud affects the bound. 


\begin{table}
\centering
\caption{Three edge scenarios}
\label{tab:delays}
\begin{tabular}{|p{1.5 cm}|p{1.7 cm}|p{1.8 cm}|p{2 cm}|}\hline
                  & Edge RTT & Remote RTT & Max edge utilization                \\ \hline
Scenario 1                      & 2 ms   & 100 ms & 95\%  \\ \hline
Scenario 2                       & 10 ms    & 30  ms   & 90\%   \\ \hline
Scenario 3             & 10 ms         & 15 ms  & 75\%     \\ \hline
\end{tabular}
\end{table}

To better understand the results, let us consider the three edge and remote cloud RTT latency scenarios summarized in Table~\ref{tab:delays}. For edge RTT latency, we consider two RTT latency values, 2 ms RTT which corresponds to the minimum expected round trip latency in future 5G networks~\cite{wp5d2017minimum}, and 10 ms RTT delay, which corresponds to the average latency expected from a 5G network when the channel is loaded~\cite{wp5d2017minimum}. For the  remote cloud RTT, we choose three values, 100 ms corresponding to a very distant remote cloud, 30 ms which corresponds to the average RTT latency we measured from our local devices to Amazon Web Services (AWS) nearest cloud data center,  and 15 ms which corresponds to previously reported values between Copenhagen and AWS's new data center in Stockholm.\footnote{As reported by Amazon https://aws.amazon.com/blogs/aws/now-open-aws-europe-stockholm-region/}
In the first scenario, the average utilization at the edge needs to be larger than 95\% for any remote cloud of any size to be beneficial, The second scenario similarly requires that the edge utilization should exceed 90\% for remote clouds to be better. For the third scenario, if the utilization at the edge exceeds 75\%, offloading computations to the remote cloud is better. We summarize these results in the fourth column of the table.

\noindent \textbf{Implications.} The first implication of our result is that the effect of the size of the remote clouds compared to an edge cloud in negligible if the size of the remote cloud is 3 orders of magnitude of the edge cloud, and if the workloads do not migrate. A typical Amazon cloud data center in 2014 had between 50000 and 80000 servers\footnote{https://www.bloomberg.com/news/2014-11-14/5-numbers-that-illustrate-the-mind-bending-size-of-amazon-s-cloud.html}. The second implication is that there will be higher resource wastage compared to a remote backend of at least 5\% when considering the first scenario, and closer to 10\% to 25\% when considering the second and third scenarios. Another solution would be to increase the amount of resources of edge clouds, making the total number of distributed servers not exactly equal to those available on a remote cloud, but larger by a factor of, e.g., 5 to 25\% to accommodate for the queuing delays. As these number represent the resources wasted for the edge cloud to have the exact same total delays compared to the remote clouds, the edge clouds will operate under even lower utilizations to make sure that the performance is not just equal, but better. 

\noindent\textbf{Implications of migrations.} The above implications do not include those resulting from application migration due to user's rapid mobility that are summarized by Equation~\ref{eq:ggsSMobi}. Migrations can severely reduce the efficacy of using an edge cloud. For example, recent state-of-the-art VM migrations and hand-off algorithms between two edges has a downtime ranging between 1.5 seconds to 6.6 seconds~\cite{chaufournier2017fast,ha2017you} making the amortized time for migration very high for applications that reside for very short number of time units. In addition, during these down times the application is completely not available, and requests arriving to the application are either queued or dropped. These delays will increase the tail response times of the applications, and  in some cases, migration can result in much higher average response times when using an edge cloud. At high edge utilization, the effect of migrations will be even higher. We nevertheless note that we expect that migration times will be reduced as VM migration technologies evolve to suit edge platforms.

\subsection{Load Skew}
\noindent\textbf{Implications.} Equations~\ref{eq:remTu} and~\ref{eq:remTu2} provide a very interesting result when it comes to VM packing on the edge cloud with many practical implications on today's virtualization trends.
Let us start by one of today's very hot trends in edge cloud virtualization, the use of serverless architectures and virtualization platforms at the edge. In the serverless model, the system uses very light weight VMs that are spawned for a very short period of time to serve a few requests before they are killed\footnote{See for example AWS's firecracker: https://firecracker-microvm.github.io/}. Running with this model would mean that in Equation~\ref{eq:remTu}, $\bar s$ would be very small, thus increasing the value of  $\frac{\rho_{edge}\tau_{edge}}{\bar s}$ considerably and affecting the overall need for an increase in the total number of edge servers drastically or even making it impossible for edge clouds to provide performance comparable to centralized large-scale clouds, without significantly increasing the edge resources. 

If  $\bar s$ is long enough though, and for the same average edge and centralized cloud load, then the average packing factor $q_{edge}$ is the only factor affecting the extra amount of resources needed by the edge cloud system to pack the same number of VMs. However, for many non-stateless computer systems, the longer an application runs, the larger its memory consumption. It is thus important to redesign the edge applications such that their resource footprint does not get bloated with time, increasing the factor $q$. We also note that, based on our results on the delay bound, when packing the VMs, the VM scheduling and admission control should take in to account the case when all of the VMs operate at maximum resource utilization, and how the increase in real system resource utilization will affect the performance at the edge. $q$ should thus be bounded based on the previous results in Section~\ref{sec:impD}.

\noindent\textbf{Implications of migrations.} Most migration algorithms today start by allocating resources at the destination edge, while still holding the resources on the source edge. This effectively reduces $q$, as a migration in essence requires, even for a brief period, double the resources of a single VM at the same time. In addition, migrations can decrease $\bar s$, if these migrations are rapid, e.g,, using serverless techniques, and $\tau_{edge}$ is large. Edge cloud capacity planners should therefore consider the frequency of migrations when initially designing the scaling factor for the edge cloud.

\subsection{The coefficient of variation}

\begin{figure*} 
\centerline{
 \subfigure[When the edge cloud server service rate is $\mu=1$, even at moderate utilization, the bound on the coefficient of variation is low.] 
{\label{fig:cv1}
\includegraphics[width=3.5 in, height=2 in]{figures/Spike_miue1s.pdf}}
  \subfigure[When the edge cloud server service rate is $\mu=10$, the bound on the coefficient of variation is high.] 
{\label{fig:cv10}
\includegraphics[width=3.5 in, height=2 in]{figures/Spike_miue10s.pdf}}
}
\caption{The bound on the coefficient of variation of the workload inter-arrival times at the edge for different $\Delta T$, when $\mu=1$ and $\mu=10$ .}
\label{fig:cv}
 \end{figure*}
 
Figures~\ref{fig:cv1} and \ref{fig:cv10} show the maximum bound on the coefficient of variation of the inter-arrival time of the workload at the edge  cloud for two different service rates, $\mu=1$ and $\mu=10$, as a function of both the edge  cloud utilization and the $\Delta T$. The bound on the coefficient of variation for the workload is a non-linear function of $\Delta T$. For smaller $\Delta T$ of up to 10 ms, the bound on the coefficient of variation of workload spikes is quite low, the workload handled can only be 4 times the average load at 60\% utilization when $\mu=1$. For the larger $\mu=10$, this increases to be 12 times the load average. We note that workload spikes can sometime be orders of magnitude more than the average workload, as typically during sport game events~\cite{ali2015analysis}.  Still, having faster servers at the edge helps with increasing the ability of edge clouds to handle the full scale of workload spikes.

\noindent\textbf{Implications.} The above result has two main system design implications. First, it is beneficial to have faster edge clouds that can serve a large number of requests per second, using for example edge accelerators~\cite{kang2017neurosurgeon} and increasing the average capacity of the edge servers. Second, these results can also guide the offloading of load from an edge cloud to a remote cloud with part of the spike served at the edge, and other parts of the spike served by the remote cloud.
This opens up many interesting resource management problems related to scheduling the workload during resource pressure between the edge and the remote cloud. From an application's design perspective, it is almost always the case that the application is in charge of choosing which parts of the computations should run locally, and which ones should be offloaded. Now, the application will need to choose when there is increased load on the the edge cloud, which computations out of the real-time latency critical requests should be offloaded even further away to the remote cloud.

\noindent \textbf{Implications of migrations.} The implications of mobility on the ability of the edge to handle spikes are summarized by equation~\ref{eq:spike1}. For smaller $\Delta T$, any increase in the  amortized time cost of a VM handover migration results in large decreases in the overall system ability to serve all requests from spikes. This decrease can be reduced by increasing the server service rates. Again, this result can be used not only to guide how to split spike workloads between edge and centralized clouds, but also to guide the decisions on VM migrations. For example, migrations, specially with larger $a$ values, can be put on hold, or only performed when the load on the receiving edge is low. Correlated migrations should be avoided so as not to be themselves a source of spikes.


% \subsection{edge  cloud design implications}


\subsection{Practical threats to validity}
While we have included many factors in our analysis, we have dropped factors that usually affect network performance. Factors such as interference, attenuation, signal reflection, multipath fading, scattering, and other complications facing communication networks, causing increased jitter, delay, or packet loss is not considered. 
In addition, it has been recently shown that many application show significantly worse tail latency than predicted by queuing models~\cite{li2014tales}. Such discrepancies can affect our analysis. However, we believe that many of these effects will face both edge and remote clouds, thus reducing their effect on our main results.
% In this section, we give some examples based on some recent studies on the delay to the edge and on the delay to a centralized cloud for both current and future networks. Table~\ref{tab:delays} summarizes these numbers from multiple studies~\cite{7842415,edgeblog}.

% Now using Equation~\ref{eq:Tau_rho}, a hard upper bound on the acceptable latency in the edge network can be calculated from the right hand side of the inequality.

% % \begin{figure*}
% % \begin{minipage}[b]{0_5\textwidth}
% % \includegraphics[width=8.5 cm]{figures/CloudDelay_serv100central25-crop.pdf}\\
% % \subcaption{Small Cluster with 100 servers at 25\% utilization.}
% % \end{minipage}%
% % \begin{minipage}[b]{0_5\textwidth}
% % \includegraphics[width=8.5 cm]{figures/CloudDelay_serv100central75-crop.pdf}\\
% % \subcaption{Small Cluster with 100 servers at 75\% utilization.}
% % \end{minipage}%
% % \newline
% % \begin{minipage}[b]{0_5\textwidth}
% % \includegraphics[width=8.5 cm]{figures/CloudDelay_serv100central95-crop.pdf}\\
% % \subcaption{Small Cluster with 100 servers at 95\% utilization.}
% % \end{minipage}%
% % \caption{For a small backend centralized cloud with only 100 servers, edge cloud resources perform relatively well until a utilization level of almost 85\%.}
% % \label{fig:SmallCloud}
% % \end{figure*}


% % \begin{figure*}
% % \begin{minipage}[b]{0_5\textwidth}
% % \includegraphics[width=8.5 cm]{figures/CloudDelay_serv1600central0-crop.pdf}\\
% % \subcaption{Medium size cloud with 1600 servers at 25\% utilization.}
% % \end{minipage}%
% % \begin{minipage}[b]{0_5\textwidth}
% % \includegraphics[width=8.5 cm]{figures/CloudDelay_serv1600central75-crop.pdf}\\
% % \subcaption{Medium size cloud with 1600 servers at 75\% utilization.}
% % \end{minipage}%
% % \newline
% % \begin{minipage}[b]{0_5\textwidth}
% % \includegraphics[width=8.5 cm]{figures/CloudDelay_serv1600central95-crop.pdf}\\
% % \subcaption{Medium size cloud with 1600 servers at 95\% utilization.}
% % \end{minipage}%
% % \caption{As the size of the backend centralized cloud increases to 1600 servers, they start to outperform the edge cloud when the edge resources utilization grows above 85\% and when the centralized cloud utilization is less than 85\%.}
% % \label{fig:midCloud}
% % \end{figure*}


% % \begin{figure*}
% % \begin{minipage}[b]{0_5\textwidth}
% % \includegraphics[width=8.5 cm]{figures/CloudDelay_serv10000central0-crop.pdf}\\
% % \subcaption{Large cloud with 10000 servers at 25\% utilization.}
% % \end{minipage}%
% % \begin{minipage}[b]{0_5\textwidth}
% % \includegraphics[width=8.5 cm]{figures/CloudDelay_serv10000central75-crop.pdf}\\
% % \subcaption{Large cloud with 10000 servers at 75\% utilization.}
% % \end{minipage}%
% % \newline
% % \begin{minipage}[b]{0_5\textwidth}
% % \includegraphics[width=8.5 cm]{figures/CloudDelay_serv10000central95-crop.pdf}\\
% % \subcaption{Large cloud with 10000 servers at 95\% utilization.}
% % \end{minipage}%
% % \caption{For a large backend centralized cloud with 10000 servers, we see a similar behaviour to the mid-sized cloud. This can already be inferred from inequality~\ref{eq:Tau_rho} as it becomes mostly dependant on $\rho_{edge}$.}
% % \label{fig:largeCloud}
% % \end{figure*}

% Figures~\ref{fig:SmallCloud},\ref{fig:midCloud} and \ref{fig:largeCloud} show the upper bounds on the RTT delay between the mobile/IoT devices and the edge cloud for three different centralized cloud sizes and for different utilization levels.
% We also plot the average RTT's from Table~\ref{tab:delays} as shown in the table---the value in the table multiplied by two.

% From the three figures, for the edge cloud service to be better than a centralized cloud, its service latency has to be smaller than the upper limit in the figures. If the utilization grows beyond 85\% on the edge, then even for small centralized clouds, the performance of the edge cloud is worse. 

% % Let us now consider the case when one wants to get a similar limit as a function of the request arrival rates and the number of servers in the system instead of utilization. Instead of using Equation\ref{eq:service} to substitute in \ref{eq:1}, we can use Equation~\ref{eq:arrival}. Thus, knowing that $s=1$ for the edge cloud case,
% % \begin{equation}
% %      \frac{\sqrt{2\lambda_{edge}}}{1-\lambda_{edge}} +\tau_{edge}< \frac{\sqrt{2\lambda_{central}}}{s-\lambda_{central}} +\tau_{central}
% % \end{equation}
% % or,
% % \begin{equation}
% %     \tau_{edge}<\frac{\sqrt{2\lambda_{central}}}{s-\lambda_{central}} +\tau_{central}-\frac{\sqrt{2\lambda_{edge}}}{1-\lambda_{edge}}.
% % \end{equation}
% % One can assume that on average $\lambda=\lambda_{edge}=\lambda_{central}/s$, therefore,
% % \begin{equation}
% % \tau_{edge}<\tau_{central}+\frac{\sqrt{2\lambda}}{\sqrt{s}(1-\lambda)} -\frac{\sqrt{2\lambda}}{1-\lambda}.
% % \end{equation}
% % % The following two commands are all you need in the
% % % initial runs of your .tex file to
% % produce the bibliography for the citations in your paper.




% % \textbf


==> skew.tex <==
\section{Edge Cloud Capacity Tradeoffs}
Having modeled and analyzed the latency tradeoffs of edge clouds, we now turn our attention to capacity tradeoffs. 
In $\S$\ref{sec:background}, we provided an intuition into why statistical multiplexing and smoothing benefits enable a centralized cloud to service the same workload as a distributed edge cloud using a smaller provisioned capacity. We model and analyze this capacity tradeoff in detail in this section.

\subsection{Modeling Edge Capacity}
Consider a distributed edge cloud with $k$ data center locations and an aggregate server capacity of $C_{edge}$ across the system. A centralized cloud services the total workload of the distributed edge cloud using a single data center with a server capacity of $C_{cloud}$. We assume that servers in the edge and centralized cloud are virtualized and resources are allocated to applications in the form of virtual machines (VMs). We assume that requests for VMs arrive according to a Poisson process with rate $\lambda$.  In the distributed edge cloud, a new VM request is assumed to be directed to the nearest edge cloud location (i.e., the one with the least distance $d$ from the user).   Requests are assumed to be uniformly distributed across the $k$ edge sites. We assume that a customer specifies a VM size (e.g., in terms of number of CPU cores) along with each  VM request. This is in line with cloud platforms that support virtual machines of different sizes. The VM size is assumed to be generally distributed. We assume $q$ to be lower bound of the number of virtual machines that can be hosted at each edge cloud site. Thus $q$ represents the VM {\em packing factor} that is a function of how many VM can be  packed onto each server and the maximum VM size that can be requested on a server.  Finally, we assume the lifetime of a VM is $\zeta$, which represents the time between a customer requesting an on-demand cloud VM and terminating it; from a queuing standpoint $\zeta$ represents the service time of a request. Then, $\bar \zeta$ and $\bar \zeta^2$ denote the mean and variance of the service times (i.e., VM lifetimes).  The utilization of each edge cloud site is given by  $\rho=\lambda \bar \zeta/k$.

We note that the problem of multiplexing virtual machines onto virtualized cloud servers has been modeled as an online bin-packing problem~\cite{wang2011consolidating,gupta2012online} and many VM placement policies based on bin packing have been proposed. Classical bin-packing is a well-studied combinatorial optimization problem \cite{CLRBook}, with recent results even allowing requests to be queued until they are placed in a bin~\cite{shah2008bin}. However, the classical model for bin-packing is not suitable for modeling an edge cloud, since in our case the arrivals of items to place in the bin is localized to a certain edge, and thus can not be placed on any other edge. In order to capture these constraints, we model the edge cloud scenario as a Dynamic Traveling Repairman Problem (DTRP), a model while popular in fields such as logistics, has not found much application in modeling computer systems.

Given the above system model, we have the following lemma for the distributed edge cloud capacity
\begin{lemma}
%The total number of servers required at the remote cloud is less than the total number of server required at the edge. 
The capacity of the edge cloud and centralized cloud are related as
 $C_{cloud} = C_{edge} \frac{(1-\rho_{edge}-\frac{\tau_{edge}}{s_{edge}})^2}{(1+1/q_{edge})(1-\rho_{cloud})^2}$
\end{lemma}
\noindent\textbf{Proof:}
VM placement in distributed edge clouds is similar to bin packing where incoming VM requests have a geographic affinity to the nearest edge cloud site.  To model capacity in such a scenario, we use a result
from the classical work of Bertsimas and Van Ryzin~\cite{bertsimas1993stochastic} where results from geometrical probability, queuing theory, and combinatorial optimization were used to obtain results on the 
{\em Dynamic Traveling Repairman Problem (DTRP)}.  In DTRP, repair requests arrive at a particular geographic locations. There are $k$  cars with repair persons that travel to the locations of repair requests, and each repair request is satisfied by the nearest car. In our case, a car (i.e., repair person) is equivalent to a
distributed edge cloud location that provides service, while a repair request is equivalent to a VM; similar to a repair request being serviced by the nearest traveling repair-person (car), VM requests are satisfied by the nearest distributed edge cloud. The DTRP analysis in  ~\cite{bertsimas1993stochastic} address the bin packing problem of how repair requests are mapped onto traveling repair persons (``bins''). The  response time $T$ (referred to as system time in ~\cite{bertsimas1993stochastic}) is the total time from the initiation of a VM request, i.e., when the user starts the upload process of the VM image to the edge site, to the time it departs (i.e., is terminated by the customer).  The analysis in ~\cite{bertsimas1993stochastic} provides packing policies for the DTRP problem with constant factor guarantees such that
\begin{equation}
    T \sim \gamma^2 \frac{\lambda A(1+1/q)^2}{C^2 v^2 (1-\rho-2\lambda \bar U/Cq)^2},  \label{eq:dtrpPack}
\end{equation}
as $\rho+\frac{2 \lambda \bar d}{v q} \longrightarrow 1$, i.e., at higher utilization and assuming $T$ is the finite response time of the packing policy (implying that VM lifetimes need to be finite). 
In this expression, $U$ is the mean time taken to upload a VM to the edge. %The velocity term $v$ represents the network bandwidth (or the upload speed of a VM) from the user to the edge cloud (or a centralized cloud) and $C$ denotes the data center capacity.


We assume that the  edge  cloud and the centralized cloud use identical packing policy, as described in~\cite{bertsimas1993stochastic}, with finite response times $T$. In this case, the utilization 
$\rho=\lambda \bar \zeta/s$, while $\tau_{edge}=2 \lambda \bar d/qv$, is the total expected upload time of the VM to the edge or the cloud.
For the edge cloud, Equation~\ref{eq:dtrpPack} is,
\begin{equation}
    T_{edge} \sim \gamma^2 \frac{\lambda A(1+1/q_{edge})^2}{C_{edge}^2 v^2 (1-\rho_{edge}-\frac{\tau_{edge}}{C_{edge}})^2},  \label{eq:edgeTu}
\end{equation}

For a centralized  cloud, with capacity $C_{cloud}$ 
since $q_{cloud}$, the number of VMs that can be packed on cloud data center before it becomes fully utilized, is very large, and is at least equal to $q_{edge}*C_{edge}$, making both $1/q$, and $\frac{\tau_{cloud}}{C_{cloud}}$ negligible. Equation~\ref{eq:dtrpPack} becomes,
\begin{equation}
    T_{cloud} \sim \gamma^2 \frac{\lambda A}{C_{cloud}^2 v^2 (1-\rho_{rem})^2}. \label{eq:remTu}
\end{equation}

If we wish to provision edge and cloud capacity such that both the distributed edge cloud and centralized 
cloud give the same packing performance under the same packing policy, 
 Equations~\ref{eq:edgeTu} and Equation~\ref{eq:remTu} need to be equal. Since both systems aim to serve the same area and the same request arrival rates, we obtain
\begin{equation}
    C_{cloud}=\frac{C_{edge}(1-\rho_{edge}-\frac{\tau_{edge}}{C_{edge}})^2}{(1+1/q_{edge})(1-\rho_{cloud})^2}. \label{eq:remTu3}
\end{equation}

\begin{corollary} \label{corr:q2} 
The capacity of the centralized cloud  needed to service the same VM workload is less than the 
that of the distributed edge cloud, that is 
$C_{cloud} < C_{edge}$
\end{corollary}
\noindent\textbf{Proof:}
Since $1-\rho_{edge}-\frac{\tau_{edge}}{C_{edge}})^2$ is necessarily less than 1 (and greater than 0), $1-\rho_{edge}-\frac{\tau_{edge}}{C_{edge}})^2 \leq 1-\rho_{cloud}$ for equivalent server utilization, and $1+1/q_{edge}$ is necessarily greater than 1, then it follows that $C_{cloud}<C_{edge}$. 

\begin{corollary} \label{corr:q}For an edge cloud data centers with a large capacity $C_{edge}$, and when the system utilization at both the edge and remote clouds are equal, $\rho_{edge}=\rho_{rem}$, then,
\begin{equation}
    \frac{C_{edge}}{C_{cloud}} = (1+1/q_{edge}). \label{eq:remTu2}
\end{equation}
\end{corollary}
\noindent\textbf{Proof:} Let the term $C_{edge}/C_{cloud}$ represent the scaling factor of the number of servers required at the edge to provide similar packing capabilities at the edge. The term $0<\rho_{edge}-\frac{\tau_{edge}}{s_{edge}}\leq1$, and if $C_{edge}$ is large enough, then $\tau_{edge}/\bar C\longrightarrow0$. The above corollary can therefore  be trivially proven.


%%%%%%%%% COMMENT OUT 

%VM multiplexing on traditional cloud servers can be modeled as an online bin-packing problem~\cite{shah2008bin,gupta2012online}. Classical bin-packing is an extremely well studied combinatorial optimization problem which aims to solve the problem of fitting a number of $n$ items of variable sizes in a minimal number of bins where the size of the items is known in advance. The online version of bin packing solves the same fitting problem, but when the item sizes are revealed one by one and each item should be placed in one of the bins as soon as its size is revealed. A more recent studied version of online packing allows the items to be queued until they are placed in a bin~\cite{shah2008bin}.
%\subsection{System Model}
%To better model multiplexing at the edge, we use the model developed by Bertsimas and Van Ryzin~\cite{bertsimas1993stochastic} in their classical work  where they combine results from geometrical probability, queuing theory and combinatorial optimization, to establish bounds on what they call the Dynamic Travelling Repairman Problem (DTRP) with multiple vehicles. DTRP is defined as follows, in a Euclidean service region with an area $A$, demand requests for a service arrive according to a Poisson process with rate $\lambda$. Demands are distributed independently and uniformly across  $A$, and are serviced by a number of vehicles $s$ that travel with a constant velocity $v$. A request is indivisible, i.e., it can not be divided on more than one vehicle. Once a vehicle arrives at the location of a service request, the service time of a request is generally distributed with a finite first and second moments---mean and variance---denoted by $\bar \zeta$ and $\bar \zeta^2$. The fraction of time spent by a vehicle on servicing requests at a site, i.e., the utilization of the vehicle, is $\rho=\lambda \bar \zeta/s$. Assuming that a vehicle can serve only $q$ customers before becoming fully utilized, they show that the \emph{optimal} minimal expected system time $T^*$ has the following lower bound:
%\begin{equation}
%    T^* \geq \frac{\gamma^2}{9} \frac{\lambda A(1+1/q)^2}{s^2 v^2 (1-\rho-2\lambda \bar d/sqv)^2}-\frac{\bar \zeta(1-2\rho)}{2 \rho},  \label{eq:dtrp}
%\end{equation}
%where, $\gamma\approx0.266$ is a constant, and $\bar d$ is the expected distance from a uniform location in A to the closest vehicle. They show that the fraction of time the server spends in radial travel, thus $2\bar d\lambda/qv$, is the time needed to reach a request. We note that the system time is the total time from the arrival of a service request until the request is serviced.
%The authors then provide packing policies $u$  that provide constant factor guarantees such that,
%\begin{equation}
%    T_u \sim \gamma_u^2 \frac{\lambda A(1+1/q)^2}{s^2 v^2 (1-\rho-2\lambda \bar d/sqv)^2},  \label{eq:dtrpPack}
%\end{equation}
%as $\rho+\frac{2 \lambda \bar d}{v q} \longrightarrow 1$, i.e., at higher utilization, where $T_u$ is the finite system time of a policy $u$.
%DTRP can be used to model the problem of edge  cloud VM multiplexing as follows.
%
%\subsection{Analytical model for VM packing}
%\begin{lemma}
%The total number of servers required at the remote cloud is less than the total number of server required at the edge. The number of servers at the remote cloud is  equal to $\frac{s_{edge}(1-\rho_{edge}-\frac{\tau_{edge}}{s_{edge}})^2}{(1+1/q_{edge})(1-\rho_{rem})^2}$.
%\end{lemma}
%\noindent\textbf{Proof:}
% We consider the service requests to be requests for hosting new VMs on one of $m_{edge}$ edge  clouds distributed across a Euclidean area $A$. The VM requests arrive according to a Poisson process with rate $\lambda$, and are distributed independently and uniformly across  $A$ such that a service request is directed to the nearest edge cloud, with the least distance $\bar d$. The velocity $v$ is then the network transfer speed (or the upload speed of a VM) from the user to the edge cloud (or a remote cloud). An edge  cloud can host a lower bound of $q$ VMs before becoming fully utilized, with no space to host other VMs. Thus, $q$ is a function of the largest VM size to be hosted on the edge. A hosted VM stays on the edge  cloud for $\bar \zeta$ time units on average with a variance of $\bar \zeta^2$. In this formulation, $\tau_{edge}=2 \lambda \bar d/qv$, is the total expected upload time of the VM to the edge or the cloud. Therefore, Equation~\ref{eq:dtrp} can be rewritten as,
%
%\begin{equation}
%    T^* \geq \frac{\gamma^2}{9} \frac{\lambda A(1+1/q)^2}{s_{edge}^2 v^2 (1-\rho-\tau_{edge}/s_{edge})^2}-\frac{\bar \zeta(1-2\rho)}{2 \rho}.
%\end{equation}
%Here, the service time of a VM request, $T^*$ is the time between the VM's intiation from the user , until its departure from either an edge cloud server or a remote cloud server. We note that here, the skew of the VM arrival rate is $1/\sqrt{\lambda}$ as the VM arrivals follow a Poisson process.
%
%In our analysis, we assume that both  edge  clouds and the remote cloud use one of the packing policies described in~\cite{bertsimas1993stochastic} with finite system times. For the edge cloud, Equation~\ref{eq:dtrpPack} is,
%
%\begin{equation}
%    T_u \sim \gamma_u^2 \frac{\lambda A(1+1/q_{edge})^2}{s_{edge}^2 v^2 (1-\rho_{edge}-\frac{\tau_{edge}}{s_{edge}})^2},  \label{eq:edgeTu}
%\end{equation}
%% but $\rho_{edge}=\lambda_{edge} \bar s/m_{edge}$, and $\tau_{edge}=2\bar r/v$, thus, 
%
%
%% \begin{equation}
%%     T_u \sim \gamma_u^2 \frac{\lambda A(1+1/q)^2}{m_{edge}^2 v^2 (1-\rho_{edge}-\rho_{edge}\tau_{edge}/\bar s)^2}. \label{eq:edgeTu}
%% \end{equation}
%
%For a remote  cloud, with $s_{rem}$ servers, 
%since $q_{rem}$, the number of VMs or user workloads that can be packed on the remote cloud before it becomes fully utilized, is very large, and is at least equal to $q_{edge}*s_{edge}$, making both $1/q$, and $\frac{\tau_{rem}}{s_{rem}}$ negligible. Equation~\ref{eq:dtrpPack} becomes,
%\begin{equation}
%    T_u \sim \gamma_u^2 \frac{\lambda A}{s_{rem}^2 v^2 (1-\rho_{rem})^2}. \label{eq:remTu}
%\end{equation}
%
%For the same packing performance, Equations~\ref{eq:edgeTu} and Equation~\ref{eq:remTu} need to be equal. Since both systems aim to serve the same area and the same request arrival rates, therefore, 
%\begin{equation}
%    s_{rem}=\frac{s_{edge}(1-\rho_{edge}-\frac{\tau_{edge}}{s_{edge}})^2}{(1+1/q_{edge})(1-\rho_{rem})^2}. \label{eq:remTu3}
%\end{equation}
%
%Since $1-\rho_{edge}-\frac{\tau_{edge}}{s_{edge}})^2$ is necessarily less than 1 (and greater than 0), $1-\rho_{edge}-\frac{\tau_{edge}}{s_{edge}})^2 \leq 1-\rho_{rem}$ for equivalent server utilization, and $1+1/q_{edge}$ is necessarily greater than 1, then it is trivial to show that $s_{rem}<s_{edge}$. 
%
%% The above result shows that, for the same utilization , and if $\rho_{edge}<1$ and $\rho_{rem}<1$ which is the necessary condition for stability when all VMs are fully utilized,  $s_{edge}/s_{rem}>1$, i.e., more resources are required to pack the same number of VMs on a system of well distributed edge clouds. The extra amount of resources needed are a function of $q_{edge}$, or the average number of VMs that can be packed on one edge cloud site, $\tau_{edge}$, and the average time a VM spends in the system $\bar s$. 
%
%\begin{corollary} \label{corr:q}For an edge cloud with a large number of edge server $s_{edge}$, and when the system utilization at both the edge and remote clouds are equal, $\rho_{edge}=\rho_{rem}$, then,
%\begin{equation}
%    \frac{s_{edge}}{s_{rem}} = (1+1/q_{edge}). \label{eq:remTu2}
%\end{equation}
%\end{corollary}
%\noindent\textbf{Proof:} Let the term $s_{edge}/s_{rem}$ represent the scaling factor of the number of servers required at the edge to provide similar packing capabilities at the edge. The term $\rho_{edge}-\frac{\tau_{edge}}{s_{edge}}<1$, and $\rho_{edge}-\rho_{edge}\tau_{edge}/\bar s\longrightarrow0$ for the minimal possible scaling factor for the edge. This will only happen if the average utilization at the edge is very low or close to zero. 
%This above corollary can therefore  be trivially proven.
%
%

%%%%%%%%%%%%%%% END COMMENT


\noindent\textbf{Discussion.} Our analytic model shows that the ability to multiplex VMs onto a larger number of servers enable a centralized cloud to be more efficient in its packing ability and require a smaller overall capacity than a distributed edge cloud to service the same workload. This property can also be illustrated through a simple example.  Suppose that each server has a unit capacity of 1, and suppose that the workload consists for placement requests for 4 VMs of capacity 0.8, 0.8, 0.2 and 0.2.  In a centralized cloud, these four VMs can be packed onto two servers, each hosting a VM of capacity 0.8 and 0.2.  In a distributed edge cloud with two sites, assuming that the first two requests arrive at the first edge location and the remaining two at the second location, we see that a total of three servers are needed---two at the first edge location, each hosting a VM of size 0.8 and one server at the second location to host two VMs, each of size 0.2.  Thus, the edge cloud needs more servers than the centralized cloud for the same workload and our analytic results provide an expression to quantify the amount of over-provisioning needed in the edge cloud with respect to the centralized cloud.  Our corollary \ref{eq:remTu2} gives a simple $(1+1/q)$ rule to quantify the amount of over-provisioning.
Since $q$ represents the VM packing factor, if we assume that each server can pack a minimum of two VMs (i.e., q=2), 
it follows the edge cloud needs a factor of 1.5 more capacity (50\% more capacity) than a centralized cloud (also illustrated in the above example). A higher packing factor $q$ and more dense packing of VMs implies  a proportionately smaller amount of edge over-provisioning. We note that these results hold for a spatially uniform distribution of VM requests across edge cloud sites. We analyze the impact of spatial skews next.




%We note that while the above results provide the amount of extra resources required for the edge to host an equivalent number of virtualized cores, i.e., for both total number of cores allocated at the edge to be equal to that of the cloud, it does not specify exactly how these extra resources should be distributed. For example, given an edge cloud system with 1000 sites, and if each site can host an average of 10 VMs, Corollary~\ref{corr:q} states that for the edge system to be equivalent to a remote cloud with 1000 servers in terms of multiplexing, the edge system should be expanded by 10\% extra resources. Simply increasing each edge site by 10\% resources does not necessarily guarantee that the total number of allocated cores for the edge system will be equivalent to the remote cloud still. This is highly dependant on the size of the VMs arriving at each site. The resulting value can thus be viewed as a lower-bound on the amount of extra capacity required at each site if the extra capacity is distributed unifromly across all sites. This result does not take in to account cases when the VM arrival rate is skewed due to geographical workload skew, which we study next. 

%  \subsection{Skew effect on request RTT}
%  \textbf{Here we discuss how load skew affects the request response time, i.e., the previous result}
 
 \subsection{Modeling Spatial Workload Skews}
 %We now turn our focus to how geographical load skews affect how efficient multiplexing can be performed on the edge. While large-scale clouds can multiplex multiple workloads, overbooking the actual resources during this multiplexing, VM multiplexing becomes harder with load skews in edge systems. We aim to quantify how much extra resources are needed to provide the edge with the same resource pooling capabilities as a remote cloud.
 
 Consider the same scenario as our previous analysis. Suppose that VM requests are no longer uniformly distributed across the $k$ edge sites and that requests have a higher probability of choosing some edge locations than others. 
 
 We extend our previous model using results from Bertsimas and Van Ryzin~\cite{bertsimas1993stochastic}. In our distributed edge cloud, we assume that VMs arrive in batches of $b$, formed due to the superposition of $r$ renewal processes (each of which is due to a certain edge customer) forming effectively a $\Sigma GI/G/s$ distributed queue. Bertsimas and Van Ryzin show that for heavy traffic, i.e., when the machines are getting close to filled, the expected waiting time for a set of VMs is 
 \begin{equation}
    E[W] \sim \frac{\lambda_{edge} (1/\lambda_{edge}^2+\sigma_s^2/k_{edge}^2}{2(1-\rho_{edge}-(\lambda_{edge}/C)(\beta(\sqrt A/(v\sqrt{b})))}, 
 \end{equation}
where $\mu_{sum}=\Sigma_j^s \mu$, $\lambda_{sum}=\Sigma_m^s \lambda$,, $\rho_{sum}=$ $ \sigma_{a_i}$ is the variance of the interarrival times of the VMs at the edge, and $ \sigma_{b_j}$ is the variance of the VM service time at the edge. We again note that here service time is equal to the time a machine resides on the edge.

However, the expected waiting time is governed by the Allen-Cunneen approximation in Equation~\ref{eq:Allen2}. We note that here the waiting time is the waiting time for a set of VMs to get placed, i.e., until there is sufficient space for the VM to be packed. Therefore, 
\begin{equation}
\begin{aligned}
  \frac{\lambda_{edge} (1/\lambda_{edge}^2+\sigma_s^2/k_{edge}^2)}{2(1-\rho_{edge}-(\lambda_{edge}/C_{edge})(\beta(\sqrt A/(v\sqrt{b}))}\sim \\ \frac{P_s/\mu_{cloud}}{1-\rho_{cloud}}.\frac{c^2_{Acloud}+c^2_{Bcloud}}{2C_{cloud}}, \label{eq:skew} 
  \end{aligned}
\end{equation}
for the same packing performance. Since we target an edge cloud with higher utilization, i.e., when servers are starting to fill up with VMs, then from equations ~\ref{eq:skew} and~\ref{eq:Bosch1},

\begin{equation}
\begin{aligned}
  \frac{\lambda_{edge} (1/\lambda_{edge}^2+\sigma_s^2/k_{edge}^2)}{2(1-\rho_{edge}-(\lambda_{edge}/C_{edge})(\beta(\sqrt A/(v\sqrt{b}))}=\\ \frac{\rho_{cloud}^2+\rho_{cloud}}{2C_{cloud}\mu_{cloud}(1-\rho_{cloud})}. \label{eq:skew2} 
  \end{aligned}
\end{equation}

\begin{corollary}
The total amount of edge capacity, $C_{edge}$, required to give the same performance a centralized cloud in the presence of geographical skews is equal to the positive root of a quadratic equation in $C_{edge}$. The root is a function of the coefficients of variations of the request arrival rate and service times at the cloud, the variance of the service time at the edge, the total number of servers in the cloud, the VM arrival rate,  the skew in VM arrival, and square root of the service area.
\end{corollary}
\noindent \textbf{Proof:} The exact quadratic equation can be obtained from Equation~\ref{eq:skew2}. It is worthwhile noting that the capacity required at the edge will be larger than that was needed when assuming no skew. The exact factor of increase is highly dependent on the skew.

\subsection{Model validation}
\noindent \textbf{Validation Setup.} In order to validate the above result, we use a real VM trace from Azure cloud services~\cite{cortez2017resource}. The dataset contains data on the arrival times, VM utilization, and sizes of over 2 Million VMs from Azure data centers in 2019. The average size of a VM is 4.75 cores, with the largest VM having 20 cores, and the smallest having 2 cores. Using the VM traces as a workload, we build a simulator that simulates edge setups of different sizes w.r.t. number of cores and/or servers per edge. The simulator is also capable of simulating remote large-scale clouds with different configurations. The simulator enables us to simulate edge sites with single, and with multiple servers, e.g., a small cluster of 10 servers with 64 cores each. This enables us to simulate different possible edge architectures, for example, some edge cloud designs suggest that each edge site should have a few racks~\cite{hilt2019future}, while others suggest an edge of a few or even a single server~\cite{choy2014hItybrid,yin2016edge}. We open source the simulator code to enable researchers to reproduce our results.\footnote{The link is redacted for blind review.}

 \begin{figure} 
\begin{center}
\includegraphics[width=3.5in]{figures/EdgeAllocPacking.png}
\end{center}
\caption{The model accurately predicts the scaling factor required between edge capacity and cloud capacity.}
\label{fig:nu}
 \end{figure}
\noindent\textbf{Validation of Corollary~\ref{eq:remTu2}.} In our first experiment, we validate the result by looking at how using our model to calculate the extra capacity required at each edge site in order to 

\begin{figure*}
\begin{minipage}[c]{0.3\linewidth}
\includegraphics[width=\linewidth]{./figures/EdgeAllocall.png}
\vspace{-0.2in}
\caption{Our model accurately predicts the number of cores/edge required for the extra resources required at the edge to pack the same number of VMs packed in the cloud.}
\label{fig:ali-mem}
\end{minipage}
\hfill
\begin{minipage}[c]{0.66\linewidth}
\centerline{
 \subfigure[Relative error for various edge configurations (cores/edge) compared to a cloud with 1000 64-core servers (Model computes 96 cores/edge).] 
{\label{fig:wikiWL} \includegraphics[width=0.45\linewidth] {figures/EdgeAlloc64.png}}
\hfill
  \subfigure[Relative error for various edge configurations (core/edge compared to a cloud with 1000 128-core servers (Model computes 160 cores/edge).] 
{\label{fig:WLTV4}\includegraphics[width=0.45\linewidth]{figures/EdgeAlloc128.png}}
}
\caption{There are diminishing returns w.r.t. the relative error compared to cloud allocation when the extra capacity is greater than what our model predicts.}
\label{fig:ali-mem-band}
\end{minipage}
\end{figure*}
 
 \noindent \textbf{Validation results.}
 
\subsection{Cost Implications}


 
%  \begin{lemma}
% Assuming equally sized edge clouds, the geographical skew in the workload requires at least $1/q_edge$ more servers compared to a backend cloud, where $q_edge$ us the number of different users who can simultaneously use the edge.
% \end{lemma}
 
 

==> xstring.tex <==
% !TeX encoding = ISO-8859-1
% Ce fichier contient le code de l'extension "xstring"
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
\def\xstringname               {xstring}                             %
\def\xstringversion              {1.83}                              %
%                                                                    %
\def\xstringdate              {2019/02/06}                           %
%                                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
% Author     : Christian Tellechea                                   %
% Status     : Maintained                                            %
% Maintainer : Christian Tellechea                                   %
% Email      : unbonpetit@netc.fr                                    %
% Package URL: https://www.ctan.org/pkg/xstring                      %
% Bug tracker: https://framagit.org/unbonpetit/xstring/issues        %
% Repository : https://framagit.org/unbonpetit/xstring/tree/master   %
% Copyright  : Christian Tellechea 2008-2019                         %
% Licence    : Released under the LaTeX Project Public License v1.3c %
%              or later, see http://www.latex-project.org/lppl.txt   %
% Files      : 1) xstring.tex                                        %
%              2) xstring.sty                                        %
%              3) xstring-fr.tex                                     %
%              4) xstring-fr.pdf                                     %
%              5) xstring-en.tex                                     %
%              6) xstring-en.pdf                                     %
%              7) README                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifdefined\usepackage\else
	\immediate\write-1 {Package: xstring \xstringdate\space v\xstringversion\space String manipulations (CT)}%
\fi
\newcount\integerpart
\newcount\decimalpart% compteurs utilisés par xstring

\edef\restorexstringcatcode{\catcode\number`\_ =\number\catcode`\_\relax}
\catcode`\_=11

\long\def\xs_execfirst#1#2{#1}
\long\def\xs_execsecond#1#2{#2}
\long\def\xs_gobarg#1{}
\expandafter\def\expandafter\xs_gobspace\space{}
\def\xs_deftok#1#2{\let#1= #2\relax}\xs_deftok\xs_sptoken{ }
\long\def\xs_ifnxttok#1#2#3{\xs_deftok\xs_toksmatch{#1}\def\__truecode{#2}\def\__falsecode{#3}\xs_ifnxttok_a}
\def\xs_ifnxttok_a{\futurelet\__futurtok\xs_ifnxttok_b}
\def\xs_ifnxttok_b{%
	\xs_ifx{\__futurtok\xs_sptoken}
		{\afterassignment\xs_ifnxttok_a\let\__futurtok= }
		{\xs_ifx{\__futurtok\xs_toksmatch}\__truecode\__falsecode}%
}
\def\xs_ifstar#1{\xs_ifnxttok*{\xs_execfirst{#1}}}
\long\def\xs_testopt#1#2{\xs_ifnxttok[{#1}{#1[{#2}]}}
\long\def\xs_exparg#1#2{\expandafter\xs_exparg_a\expandafter{#2}{#1}}%
\long\def\xs_exparg_a#1#2{#2{#1}}
\long\def\xs_exptwoargs#1#2#3{\xs_exparg{\xs_exparg{#1}{#2}}{#3}}
\long\def\xs_eearg#1#2{\xs_exparg{\xs_exparg{#1}}{#2}}
\long\def\xs_edefaddtomacro#1#2{\edef#1{\unexpanded\expandafter{#1}#2}}
\long\def\xs_addtomacro#1#2{\xs_exparg{\def#1}{#1#2}}
\long\def\xs_eaddtomacro#1#2{\xs_exparg{\xs_addtomacro#1}{#2}}
\long\def\xs_eeaddtomacro#1#2{\xs_exparg{\xs_eaddtomacro#1}{#2}}
\long\def\xs_endgroup_eaddtomacro#1#2{\xs_exparg{\endgroup\xs_addtomacro#1}{#2}}
\long\def\xs_beforespace#1 #2\_nil{#1}
\long\def\xs_afterspace#1 #2\_nil{#2}
\long\def\xs_gobtonil#1\_nil{}
\long\def\xs_gobtobrace#1#{}
\long\def\xs_ifx#1{\ifx#1\expandafter\xs_execfirst\else\expandafter\xs_execsecond\fi}
\def\xs_ifnum#1{\ifnum#1\expandafter\xs_execfirst\else\expandafter\xs_execsecond\fi}
\long\def\xs_ifempty#1{\expandafter\xs_ifx\expandafter{\expandafter\relax\detokenize{#1}\relax}}

\def\xs_toks_toverb{% lit 1 argument et le transforme en verb
	\begingroup
		\def\do##1{\catcode`##112 }%
		\dospecials
		\obeyspaces
		\xs_read_verb
}

\def\setverbdelim#1{% définit quel est le délimiteur de verb
	\xs_exparg\xs_ifempty{\xs_gobarg#1}%
		{}
		{\errmessage{Package xstring Warning: verb delimiter "\detokenize{#1}" is not a single token}}%
	\def\xs_read_verb##1#1##2#1{\endgroup\xs_assign_verb{##2}}% on appelle l'exécution de fin
}

% Assigne l'argument entre délimiteur verb dans la sc #1
\def\verbtocs#1{%
	\def\xs_assign_verb##1{\def#1{##1}}%
	\xs_toks_toverb
}

\begingroup
	\catcode0 3 \gdef\xs_twozeroschars{^^00}%
	\catcode0 7 \xdef\xs_twozeroschars{\xs_twozeroschars^^00}%
\endgroup

\edef\xs_reserved_A{\long\def\noexpand\xs_assigntokenizeresult##1\xs_twozeroschars}
\xs_reserved_A#2{\endgroup\xs_exparg{\def#2}{\xs_gobarg#1}}

\def\tokenize#1#2{%
	\begingroup
		\xs_def\xs_reserved_A{#2}% on développe en accord avec \fullexpandarg ou \noexpandarg
		\everyeof\expandafter{\xs_twozeroschars#1}%
		\endlinechar-1
		\expandafter\xs_assigntokenizeresult\scantokens\expandafter{\expandafter\relax\xs_reserved_A}% on fait l'assignation
}%

\long\def\xs_assign_xstringresult#1#2{\xs_ifempty{#2}{#1}{\def#2{#1}}}

\def\xs_ldef{\long\def}
\def\xs_ledef{\long\edef}

\def\normalexpandarg{%
	\let\xs_def\xs_ldef% on définit \xs_call avec \def
	\def\xs_expand##1{\unexpanded\expandafter{##1}}%
}
\let\noexpandarg\normalexpandarg% synonyme

\def\expandarg{%
	\let\xs_def\xs_ldef% on définit \xs_call avec \def
	\def\xs_expand##1{\unexpanded\expandafter\expandafter\expandafter{##1}}%
}

\def\fullexpandarg{%
	\let\xs_def\xs_ledef% on définit\xs_call avec \edef
	\def\xs_expand##1{##1}% et on neutralise \xs_expand
}

\def\saveexpandmode{\let\xs_saved_def\xs_defarg\let\xs_saved_expand\xs_expand}
\def\restoreexpandmode{\let\xs_defarg\xs_saved_def\let\xs_expand\xs_saved_expand}

% Macro interne renvoyant #2 si son argument commence par une accolade ouvrante "{"
% et #3 sinon (Ulrich Diez sur comp.text.tex)
\long\def\xs_ifbeginwithbrace#1{%
	\csname xs_exec%
		\expandafter\xs_gobarg\string{%
		\expandafter\xs_gobarg\expandafter{\expandafter{\string#1}%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\xs_execfirst
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\xs_gobarg
		\expandafter\expandafter\expandafter\xs_gobarg
		\expandafter\expandafter\expandafter{\expandafter\string\expandafter}\string}%
		\expandafter\xs_gobarg\string}%
		\xs_execsecond{first}{second}%
	\endcsname
}

% Cette macro interne prend la 1ere unité syntaxique de #1 et assigne le résultat à #2
\long\def\xs_returnfirstsyntaxunit#1#2{%
	\let\xs_toks\relax
	\xs_ifempty{#1}
		{\let#2\empty
		}
		{\xs_eearg\xs_ifempty{\expandafter\xs_beforespace\detokenize{#1} \_nil}% #1 commence par un espace ?
			{\def#2{ }}
			{\xs_ifbeginwithbrace{#1}
				{\def\xs_groupfound{\xs_exparg{\def#2}{\expandafter{#2}}\xs_gobtonil}% on met #2 dans des accolades et on finit
				\let\xs_toks\bgroup
				\afterassignment\xs_groupfound
				\def#2%
				}
				{\long\def\xs_assignfirstarg##1##2\_nil{\def#2{##1}}%
				\xs_assignfirstarg
				}%
			#1\_nil
			}%
		}%
}

\long\def\xs_removefirstsyntaxunit#1#2{%
	\xs_ifempty{#1}
		{\let#2\empty
		}
		{\xs_eearg\xs_ifempty{\expandafter\xs_beforespace\detokenize{#1} \_nil}% #1 commence par un espace ?
			{\xs_exparg\xs_ifbeginwithbrace{\xs_gobspace#1}
				{\xs_exparg{\def#2}{\xs_gobtobrace#1}}%
				{\xs_exparg{\def#2}{\xs_afterspace#1\_nil}}%
			}%
			{\xs_exparg{\def#2}{\xs_gobarg#1}}%
		}%
}

% Cette macro interne est utilisée dans les macros étoilées pour :
% 1) développer l'argument selon qu'on a choisit \fullexpandarg
%    ou \normalexpandarg, et ceci à l'aide de la macro \xs_def
% 2) Ensuite, on détokenize ce développement de façon n'avoir plus que
%    des catcodes de 10 pour les espaces et 12 pour le reste.
\long\def\xs_expand_and_detokenize#1#2{%
	\long\def#1{#2}%
	\expandafter\edef\expandafter#1\expandafter{\xs_expand#1}% on développe #2 selon le mode de développement
	\long\edef#1{\detokenize\expandafter{#1}}% puis on détokenize et on assigne à #1
}

\long\def\xs_expand_and_assign#1#2{\xs_def#1{#2}}% on développe #2 selon \fullexpandarg ou \normalexpandarg

\def\xs_arglist{0########1########2########3########4########5########6########7########8########9}

% \xs_assign_args{3} met dans la sc \xs_myarg les tokens "####1####2####3"
\def\xs_assign_args#1{\def\xs_assign_args_i0##1#1##2\_nil{\def\xs_myarg{##1#1}}\expandafter\xs_assign_args_i\xs_arglist\_nil}

% \xs_assign_opt_args{3} met dans la sc \xs_myarg les tokens "[####1]####2####3####4"
\def\xs_assign_opt_args#1{\xs_exparg\xs_assign_opt_args_i{\number\numexpr#1+1}}
\def\xs_assign_opt_args_i#1{\def\xs_assign_opt_args_ii0##11##2#1##3\_nil{\def\xs_myarg{[##11]##2#1}}\expandafter\xs_assign_opt_args_ii\xs_arglist\_nil}

% \xs_assign_one_arg{3} met dans la sc \xs_myarg les tokens "####3"
\def\xs_assign_one_arg#1{\xs_exparg\xs_assign_one_arg_i{\number\numexpr#1-1}{#1}}
\def\xs_assign_one_arg_i#1#2{\def\xs_assign_one_arg_ii##1#1##2#2##3\_nil{\def\xs_myarg{##2#2}}\expandafter\xs_assign_one_arg_ii\xs_arglist\_nil}

% #1 : numéro du 1er argument; #2 : nombre de lignes; #3 argument optionnel; #4 : dernier numéro de l'argument devant être détokenisé si étoile
\def\xs_buildlines#1#2#3#4{%
	\let\xs_newlines\empty
	\let\xs_newargs\empty
	\def\xs_buildlines_i##1{%
		\xs_exparg\xs_assign_one_arg{\number\numexpr##1+#1-1}%
		\edef\xs_reserved_B{\noexpand\xs_expand\csname xs_arg_\romannumeral\numexpr##1\endcsname}%
		\xs_ifnum{##1=1 }% si c'est le premier argument
			{\xs_ifempty{#3}%
				{\xs_eaddtomacro\xs_newargs{\expandafter{\xs_reserved_B}}%
				\edef\xs_reserved_B{\ifnum##1>#4 xs_def\else xs_assign\fi}%
				}% et s'il y a un argument optionnel alors, on met des crochets
				{\xs_eaddtomacro\xs_newargs{\expandafter[\xs_reserved_B]}%
				\def\xs_reserved_B{xs_def}% ne pas détokéniser l'argument optionnel grace au \xs_def
				}%
			}
			{\xs_eaddtomacro\xs_newargs{\expandafter{\xs_reserved_B}}%
			\edef\xs_reserved_B{\ifnum##1>#4 xs_def\else xs_assign\fi}%
			}%
		\edef\xs_newlines{\unexpanded\expandafter{\xs_newlines}\expandafter\noexpand\csname\xs_reserved_B\endcsname\expandafter\noexpand\csname xs_arg_\romannumeral\numexpr##1\endcsname{\xs_myarg}}%
		\xs_ifnum{##1<#2 }
			{\xs_exparg\xs_buildlines_i{\number\numexpr##1+1}}
			{}%
	}%
	\xs_buildlines_i1%
}

\def\xs_newmacro{%
	\xs_ifstar
		{\let\xs_reserved_D\empty\xs_newmacro_}
		{\let\xs_reserved_D\relax\xs_newmacro_0}%
}

% #1 : dernier numéro de l'argument devant être détokenisé
% #2 : nom de la macro publique
% #3 : argument optionnel (vide si pas d'arg optionnel)
% #4 : nombre d'arguments obligatoires
% #5 : utilisation de testopt (1 si oui, 0 si non)
% #6 : code de la macro
\def\xs_newmacro_#1#2#3#4#5{%
	\edef\xs_reserved_A{xs_\expandafter\xs_gobarg\string#2}%
	\edef\xs_reserved_C{\expandafter\noexpand\csname\xs_reserved_A _\ifx\empty#3\empty _\fi\endcsname}%
	\edef\xs_reserved_B{%
		\long
		\ifx\empty\xs_reserved_D
			\def\noexpand#2{\noexpand\xs_ifstar
				{\let\noexpand\xs_assign\noexpand\xs_expand_and_detokenize\expandafter\noexpand\xs_reserved_C}%
				{\let\noexpand\xs_assign\noexpand\xs_expand_and_assign\expandafter\noexpand\xs_reserved_C}%
			}%
		\else
			\def\noexpand#2{\let\noexpand\xs_assign\noexpand\xs_expand_and_assign\expandafter\noexpand\xs_reserved_C}%
		\fi
		\ifx\empty#3\empty
		\else
			\def\expandafter\noexpand\xs_reserved_C{%
				\noexpand\xs_testopt{\expandafter\noexpand\csname\xs_reserved_A __\endcsname}{\ifx\xs_def\xs_ledef#3\else\unexpanded{#3}\fi}}%
		\fi
	}%
	% Que fait \xs_reserved_B ? Il définit :
	% si #3 est vide : \NOM{\xs_ifstar{\let\xs_assign\xs_expand_and_detokenize\xs_NOM__}{\let\xs_assign\xs_expand_and_assign\xs_NOM__}}
	% si #3 existe   : \NOM{\xs_ifstar{\let\xs_assign\xs_expand_and_detokenize\xs_NOM_}{\let\xs_assign\xs_expand_and_assign\xs_NOM_}}
	%                  \xs_NOM_{\xs_testopt{\xs_NOM__}{#3}}}
	\xs_reserved_B
	\ifx\empty#3\empty
		\xs_buildlines1{#4}{#3}{#1}%
		\xs_assign_args{#4}%
	\else
		\xs_exparg{\xs_buildlines1}{\number\numexpr#4+1}{#3}{#1}%
		\xs_assign_opt_args{#4}%
	\fi
	\edef\xs_reserved_B{\def\expandafter\noexpand\csname\xs_reserved_A __\endcsname\xs_myarg}%
	\edef\xs_reserved_C{\unexpanded\expandafter{\xs_newlines}\edef\noexpand\xs_call}%
	\edef\xs_reserved_D{\noexpand\noexpand\expandafter\noexpand\csname\xs_reserved_A\endcsname\unexpanded\expandafter{\xs_newargs}}%
	\ifnum#5=1 \edef\xs_reserved_D{\noexpand\noexpand\noexpand\xs_testopt{\unexpanded\expandafter{\xs_reserved_D}}{}}\fi
	\xs_edefaddtomacro\xs_reserved_C{{\unexpanded\expandafter{\xs_reserved_D}}\noexpand\xs_call}%
	\xs_edefaddtomacro\xs_reserved_B{{\unexpanded\expandafter{\xs_reserved_C}}}%
	% Que fait \xs_reserved_B ? Il définit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def\xs_NOM__[##2]##3##4##5{%
	%          \xs_def\xs_arg_i{##2}\xs_assign\xs_arg_ii{##3}\xs_assign\xs_arg_iii{##4}\xs_asign\xs_arg_iv{##5}%
	% si #5=0: \edef\xs_call{\noexpand\xs_NOM[\xs_expand\xs_arg_i]{\xs_expand\xs_arg_ii}{\xs_expand\xs_arg_iii}{\xs_expand\xs_arg_iv}}%
	% si #5=1: \edef\xs_call{\noexpand\xs_testopt{\noexpand\xs_NOM[\xs_expand\xs_arg_i]{\xs_expand\xs_arg_i}{\xs_expand\xs_arg_ii}{\xs_expand\xs_arg_iii}{\xs_expand\xs_arg_iv}}{}}%
	%          \xs_call}
	\long\xs_reserved_B
	\edef\xs_reserved_B{%
		\def\expandafter\noexpand\csname\xs_reserved_A\endcsname
			\xs_myarg\ifnum#5=1 [\unexpanded{##}\number\numexpr\ifx\empty#3\empty#4+1\else#4+2\fi]\fi
	}%
	% Que fait \xs_reserved_B ? Il définit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def \xs_NOM[##2]##3##4##5[##6]{#6}
	\long\xs_reserved_B
}

% macro générique qui lit \xs_reserved_C us par us
% 3 sous-routines sont appelées à des moments clé :
% \xs_atendofgroup      (un groupe se finit, appel récursif)
% \xs_atbegingroup      (un groupe vient d'être ouvert)
% \xs_atnextsyntaxunit  (la future US n'est pas un groupe)
\def\xs_read_reserved_C{%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
		{\xs_ifnum{\xs_nestlevel=0 }
			{}
			{\xs_atendofgroup
			\xs_read_reserved_C
			}%
		}
		{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_A
		\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
		\xs_exploregroups
		\xs_ifx{\bgroup\xs_toks}
			{\advance\integerpart1
			\begingroup
				\expandafter\def\expandafter\xs_reserved_C\xs_reserved_A
				\xs_calc_grouIP
				\def\xs_nestlevel{1}%
				\integerpart0
				\xs_atbegingroup
			}
			{\advance\decimalpart1
			\xs_atnextsyntaxunit
			}%
		\xs_read_reserved_C
		}%
}

% macro générique qui lit \xs_reserved_D en procédant à des tests avec \IfBeginWith
% 1 sous-routine est appelée :
% \xs_atoccurfound      (une occurrence a été trouvée)
\def\xs_read_reserved_D{%
	\xs_exparg\xs_ifempty{\xs_reserved_D}%
		{\xs_ifnum{\xs_nestlevel=0 }
			{}
			{\edef\__temp{%
				\endgroup
				\noexpand\decimalpart=\number\decimalpart\relax
				\unexpanded{\xs_addtomacro\xs_reserved_C}{{\unexpanded\expandafter{\xs_reserved_C}}}%
				}%
			\__temp
			\xs_read_reserved_D
			}%
		}%
		{\xs_exptwoargs\xs_IfBeginWith_i\xs_reserved_D\xs_reserved_E
			{\advance\decimalpart1
			\let\xs_reserved_D\xs_reserved_A
			\xs_atoccurfound
			}%
			{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_D}\xs_reserved_A
			\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_D}\xs_reserved_D
			\xs_exploregroups
			\xs_ifx{\bgroup\xs_toks}
				{\advance\integerpart1
				\begingroup
					\expandafter\def\expandafter\xs_reserved_D\xs_reserved_A
					\xs_calc_grouIP
					\let\xs_reserved_C\empty
					\def\xs_nestlevel{1}%
					\integerpart0
				}
				{\xs_eaddtomacro\xs_reserved_C{\xs_reserved_A}%
				}%
			}%
		\xs_read_reserved_D
		}%
}

\xs_newmacro\StrRemoveBraces{}{1}{1}{%
	\def\xs_reserved_C{#1}%
	\let\xs_reserved_B\empty
	\def\xs_nestlevel{0}%
	\xs_StrRemoveBraces_i
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#2}%
}

\def\xs_StrRemoveBraces_i{%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
		{\xs_ifnum{\xs_nestlevel=0 }
			{}
			{\xs_endgroup_eaddtomacro\xs_reserved_B\xs_reserved_B
			\xs_StrRemoveBraces_i
			}%
		}
		{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_A
		\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
		\xs_ifx{\bgroup\xs_toks}
			{\xs_ifx{\xs_exploregroups\relax}% on explore les groupes ?
				{\begingroup
					\expandafter\def\expandafter\xs_reserved_C\xs_reserved_A
					\def\xs_nestlevel{1}%
					\let\xs_reserved_B\empty
				}
				{\expandafter\xs_addtomacro\expandafter\xs_reserved_B\xs_reserved_A
				}%
			}
			{\xs_eaddtomacro\xs_reserved_B{\xs_reserved_A}%
			}%
		\xs_StrRemoveBraces_i
		}%
}

% \xs_cutafteroccur coupe l'argument #1 après la #3ème occurrence de #2
% \xs_reserved_C : contient ce qui se trouve avant cette occurrence
% \xs_reserved_D : contient ce qui se trouve avant cette occurrence y compris cette occurrence
% \xs_reserved_E : contient ce qui se trouve après l'occurrence
% si l'occurrence n'existe pas ou qu'un des arguments est vide, toutes les chaines renvoyées sont vides
\long\def\xs_cutafteroccur#1#2#3{%
	\xs_ifnum{#3<1 }
		{\let\xs_reserved_C\empty\let\xs_reserved_E\empty\gdef\groupID{}}
		{\xs_cutafteroccur_i{#1}{#2}{#3}}%
}
	
\long\def\xs_cutafteroccur_i#1#2#3{%
	\def\xs_reserved_D{#1}\let\xs_reserved_C\empty\def\xs_reserved_E{#2}%
	\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
	\def\xs_atoccurfound{%
		\xs_ifnum{\decimalpart=\numexpr(#3)\relax}
			{\edef\__temp{%
				\def\noexpand\xs_reserved_C{\unexpanded\expandafter{\xs_reserved_C}}%
				\def\noexpand\xs_reserved_D{\unexpanded\expandafter{\xs_reserved_D}}%
				\noexpand\decimalpart=\number\decimalpart\relax
				}%
			\expandafter\xs_exitallgroups\__temp
			\xs_gobarg% mange l'appel récursif \xs_read_reserved_D dans \xs_read_reserved_D
			}
			{\xs_eaddtomacro\xs_reserved_C{\xs_reserved_E}%
			}%
	}%
	\xs_read_reserved_D
	\xs_ifnum{\decimalpart=\numexpr(#3)\relax}% occurrence trouvée ?
		{\let\xs_reserved_E\xs_reserved_D
		\xs_exparg{\def\xs_reserved_D}{\xs_reserved_C#2}%
		}
		{\let\xs_reserved_C\empty
		\let\xs_reserved_E\empty
		\gdef\groupID{}%
		}%
}

\xs_newmacro*3\IfSubStr{1}{2}{0}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\xs_exparg\xs_ifempty{\xs_reserved_D}\xs_execsecond\xs_execfirst
}

\xs_newmacro*2\IfBeginWith{}{2}{0}{%
	\xs_ifempty{#2}%
		{\xs_execsecond}
		{\xs_IfBeginWith_i{#1}{#2}}%
}

\long\def\xs_IfBeginWith_i#1#2{%
	\xs_ifempty{#2}%
		{\xs_execfirst% #2 est vide, tous les tests sont passés avec succès : on renvoie #3
		}
		{\xs_ifempty{#1}%
			{\xs_execsecond% #1 est vide, c'est que #2 est + long que #1 : on renvoie #4
			}
			{\xs_returnfirstsyntaxunit{#2}\xs_reserved_B
			\xs_returnfirstsyntaxunit{#1}\xs_reserved_A
			\xs_ifx{\xs_reserved_A\xs_reserved_B}% il y a égalité...
				{\xs_removefirstsyntaxunit{#2}\xs_reserved_B
				\xs_removefirstsyntaxunit{#1}\xs_reserved_A% on enlève les 1ere unités syntaxiques
				\xs_exptwoargs\xs_IfBeginWith_i\xs_reserved_A\xs_reserved_B
				}
				{\xs_execsecond
				}%
			}%
		}%
}

\xs_newmacro*2\IfEndWith{}{2}{0}{%
	\xs_ifempty{#2}%
		{\xs_execsecond
		}
		{\xs_StrCount{#1}{#2}[\xs_reserved_A]%
		\xs_ifnum{\xs_reserved_A=0 }
			{\xs_execsecond}
			{\xs_exparg\xs_ifempty{\xs_reserved_C}}%
		}%
}

\xs_newmacro*4\IfSubStrBefore{1,1}{3}{0}{\xs_IfSubStrBefore_i[#1]{#2}{#3}{#4}}

\def\xs_IfSubStrBefore_i[#1,#2]#3#4#5{%
	\def\xs_reserved_C{#3}%
	\xs_ifx{\xs_exploregroups\relax}% si on explore les groupes
		{\let\xs_reserved_B\empty
		\def\xs_nestlevel{0}%
		\xs_StrRemoveBraces_i% on retire les accolades
		\let\xs_reserved_C\xs_reserved_B
		}
		{}%
	\xs_exparg\xs_cutafteroccur\xs_reserved_C{#5}{#2}%
	\xs_exparg\xs_cutafteroccur\xs_reserved_C{#4}{#1}%
	\gdef\groupID{}%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
		\xs_execsecond
		\xs_execfirst
}

\xs_newmacro*4\IfSubStrBehind{1,1}{3}{0}{\xs_IfSubStrBehind_i[#1]{#2}{#3}{#4}}
\long\def\xs_IfSubStrBehind_i[#1,#2]#3#4#5{\xs_IfSubStrBefore_i[#2,#1]{#3}{#5}{#4}}

\long\def\xs_formatnumber#1#2{%
	\xs_ifempty{#1}%
		{\def#2{0X}% si vide, renvoie 0X
		}
		{\xs_returnfirstsyntaxunit{#1}\xs_reserved_A
		\def\xs_reserved_B{+}%
		\xs_ifx{\xs_reserved_A\xs_reserved_B}
			{\xs_removefirstsyntaxunit{#1}\xs_reserved_C
			\xs_exparg\xs_ifempty{\xs_reserved_C}%
				{\def#2{+0X}}
				{\xs_exparg{\def#2}{\expandafter+\expandafter0\xs_reserved_C}}%
			}
			{\def\xs_reserved_B{-}%
			\xs_ifx{\xs_reserved_A\xs_reserved_B}
				{\xs_removefirstsyntaxunit{#1}\xs_reserved_A
				\xs_exparg\xs_ifempty{\xs_reserved_A}%
					{\def#2{-0X}}%
					{\xs_exparg{\def#2}{\expandafter-\expandafter0\xs_reserved_A}}%
				}
				{\def#2{0#1}%
				}%
			}%
		}%
}

\xs_newmacro\IfInteger{}{1}{0}{%
	\xs_formatnumber{#1}\xs_reserved_A
	\decimalpart0
	\afterassignment\xs_defafterinteger\integerpart\xs_reserved_A\relax\_nil
	\let\xs_after_intpart\afterinteger
	\expandafter\xs_testdot\afterinteger\_nil
	\xs_ifx{\empty\afterdecimal}
		{\xs_ifnum{\decimalpart=0 }
			{\xs_execfirst% partie décimale constituée de 0 --> seul cas où on renvoie vrai
			}
			{\expandafter\xs_defafterinteger\xs_after_intpart\relax\_nil
			\xs_execsecond
			}%
		}
		{\expandafter\xs_defafterinteger\xs_after_intpart\relax\_nil
		\xs_execsecond
		}%
}

\xs_newmacro\IfDecimal{}{1}{0}{%
	\xs_formatnumber{#1}\xs_reserved_A
	\decimalpart0
	\afterassignment\xs_defafterinteger\integerpart\xs_reserved_A\relax\_nil
	\expandafter\xs_testdot\afterinteger\_nil
	\xs_ifx{\empty\afterdecimal}
}

\begingroup\catcode`\@ 11
\long\gdef\xs_defafterinteger#1\relax\_nil{\def\@xs@afterinteger{#1}\let\afterinteger\@xs@afterinteger}
\long\gdef\xs_defafterdecimal#1\_nil{\def\@xs@afterdecimal{#1}\let\afterdecimal\@xs@afterinteger}
\endgroup

\def\xs_testdot{%
	\let\xs_decsep\empty
	\xs_ifnxttok.
		{\def\xs_decsep{.}\xs_readdecimalpart}%
		{\xs_testcomma}%
}

\def\xs_testcomma{%
	\xs_ifnxttok,
		{\def\xs_dessep{,}\xs_readdecimalpart}%
		{\xs_defafterdecimal}%
}

\long\def\xs_readdecimalpart#1#2\_nil{%
	\xs_ifempty{#2}
		{\def\xs_reserved_A{0X}}
		{\def\xs_reserved_A{0#2}}%
	\afterassignment\xs_defafterinteger\decimalpart\xs_reserved_A\relax\_nil
	\expandafter\xs_defafterdecimal\afterinteger\_nil
}

% test d'égalité sur des chaines (et des chaines contenant des nombres)
\long\def\xs_IfStrEqFalse_i#1#2{\let\xs_reserved_A\xs_execsecond}
\long\def\xs_IfStrEqFalse_ii#1#2{% renvoie vrai si les 2 arg sont décimaux et s'ils sont égaux, faux sinon
	\xs_IfDecimal{#1}%
		{\xs_IfDecimal{#2}%
			{\ifdim#1pt=#2pt
				\let\xs_reserved_A\xs_execfirst
			\else
				\let\xs_reserved_A\xs_execsecond
			\fi% les 2 sont décimaux : on fait le test
			}%
			{\let\xs_reserved_A\xs_execsecond}% un seul est décimal
		}%
		{\let\xs_reserved_A\xs_execsecond}% #1 n'est pas décimal
}

\long\def\xs_TestEqual#1#2{% teste si les 2 arguments sont égaux
	\def\xs_reserved_A{#1}\def\xs_reserved_B{#2}%
	\xs_ifx{\xs_reserved_A\xs_reserved_B}
		{\let\xs_reserved_A\xs_execfirst}% égalité parfaite des 2 chaines
		{\xs_reserved_D{#1}{#2}}%
	\xs_reserved_A
}

\xs_newmacro*2\IfStrEq{}{2}{0}{% teste si les deux chaines sont égales
	\let\xs_reserved_D\xs_IfStrEqFalse_i
	\xs_TestEqual{#1}{#2}%
}

\xs_newmacro*2\IfEq{}{2}{0}{% teste si les 2 arguments (chaine ou nombre) sont égaux
	\let\xs_reserved_D\xs_IfStrEqFalse_ii
	\xs_TestEqual{#1}{#2}%
}

\def\IfStrEqCase{%
	\xs_ifstar
		{\xs_IfStringCase{\IfStrEq*}}%
		{\xs_IfStringCase\IfStrEq}%
}

\def\IfEqCase{%
	\xs_ifstar
		{\xs_IfStringCase{\IfEq*}}%
		{\xs_IfStringCase\IfEq}%
}

\long\def\xs_IfStringCase#1#2#3{% #1=macro avec ou sans étoile  #2=argument à tester  #3=liste des {<cas>}{code>}
	\long\def\xs_testcase##1##2##3\_nil{% lit les 2 premieres unités syntaxiques dans ##1 et ##2. Les autres dans ##3
		#1{#2}{##1}% compare
			{\xs_testopt{\xs_IfStringCase_ii{##2}}{}}% le test est positif, on exécute le code correspondant et on mange l'argument optionnel ## BUGfix dans 1.82
			{\xs_ifempty{##3}%
				{\xs_testopt{\xs_IfStringCase_i}{}}% s'il n'y a plus de cas, on exécute le code <autres cas> ## BUGfix dans 1.82
				{\xs_testcase##3\_nil}% sinon, on recommence avec ce qui reste
			}%
	}%
	\xs_testcase#3\_nil
}

\long\def\xs_IfStringCase_i[#1]{#1}
\long\def\xs_IfStringCase_ii#1[#2]{#1}

% Renvoie ce qui est à gauche de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\xs_newmacro*3\StrBefore{1}{2}{1}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#4}%
}

% Renvoie ce qui est à droite de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\xs_newmacro*3\StrBehind{1}{2}{1}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_E}{#4}%
}

% Renvoie ce qui est strictement compris entre les occurrences n°#1 et n°#2
% des chaines #4 et #5 dans la chaine #3
\xs_newmacro*4\StrBetween{1,1}{3}{1}{\xs_StrBetween_i[#1]{#2}{#3}{#4}[#5]}
\long\def\xs_StrBetween_i[#1,#2]#3#4#5[#6]{%
	\begingroup
		\noexploregroups
		\xs_cutafteroccur{#3}{#5}{#2}%
		\xs_exparg\xs_cutafteroccur{\xs_reserved_C}{#4}{#1}%
		\expandafter
	\endgroup
	\expandafter\xs_assign_xstringresult\expandafter{\xs_reserved_E}{#6}%
	\gdef\groupID{}%
}

\def\exploregroups{\let\xs_exploregroups\relax}
\def\noexploregroups{\def\xs_exploregroups{\let\xs_toks\relax}}
\def\saveexploremode{\let\xs_saveexploremode\xs_exploregroups}
\def\restoreexploremode{\let\xs_exploregroups\xs_saveexploremode}

% Remplace les #1 premières occurences de la chaine #3
% par la chaine #4 dans la chaine #2
\xs_newmacro\StrSubstitute{0}{3}{1}{%
	\def\xs_reserved_D{#2}\let\xs_reserved_C\empty\def\xs_reserved_E{#3}%
	\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
	\def\xs_atoccurfound{%
		\xs_ifnum{#1<1 }
			{\def\xs_reserved_A{#4}}
			{\xs_ifnum{\decimalpart>#1 }
				{\def\xs_reserved_A{#3}}
				{\def\xs_reserved_A{#4}}%
			}%
		\xs_eaddtomacro\xs_reserved_C{\xs_reserved_A}%
	}%
	\xs_ifempty{#3}%
		{\xs_exparg\xs_assign_xstringresult{\xs_reserved_D}{#5}%
		}
		{\xs_read_reserved_D
		\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#5}%
		}%
}

% Supprime les #1 premières occurrences de #3 dans #2
\xs_newmacro\StrDel{0}{2}{1}{\xs_StrSubstitute[#1]{#2}{#3}{}[#4]}

\def\xs_exitallgroups{\ifnum\xs_nestlevel>0 \endgroup\expandafter\xs_exitallgroups\fi}

% Compte combien d'unités syntaxiques contient la chaine #1 ?
\xs_newmacro\StrLen{}{1}{1}{%
	\def\xs_reserved_C{#1}\decimalpart0 \def\xs_nestlevel{0}\gdef\groupID{0}%
	\let\xs_atbegingroup\relax
	\def\xs_atendofgroup{\expandafter\endgroup\expandafter\decimalpart\number\decimalpart\relax}%
	\let\xs_atnextsyntaxunit\relax
	\xs_read_reserved_C
	\xs_exparg\xs_assign_xstringresult{\number\decimalpart}{#2}%
}

% Macro interne fermant autant de groupes que nécessaire pour trouver une unité syntaxique derrière
\def\xs_continuetonext{%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
		{\ifnum\xs_nestlevel>0
			\xs_endgroup_eaddtomacro\xs_reserved_B{\expandafter{\xs_reserved_B}}% on concatène
			\expandafter\xs_continuetonext% on recommence
		\fi}
		{}%
}%

\def\xs_calc_grouIP{%
	\begingroup\def\xs_reserved_A{0}%
	\xs_ifx{\xs_reserved_A\groupID}% si on arrive du groupe de niveau 0
		{\endgroup\xdef\groupID{\number\integerpart}}% on met simplement le niveau
		{\endgroup\xs_eearg{\gdef\groupID}{\expandafter\groupID\expandafter,\number\integerpart}}%
}

% Cette macro coupe la chaine #1 après l'unité syntaxique n°#2
\def\StrSplit{%
	\xs_ifstar
		{\let\xs_reserved_E\xs_continuetonext\StrSplit_i}%
		{\let\xs_reserved_E\relax\StrSplit_i}%
}

\xs_newmacro\StrSplit_i{}{2}{0}{\xs_StrSplit_ii{#2}{#1}\xs_StrSplit_iii}

% Cette macro interne coupe la chaine #2 après l'unité syntaxique n°#1
% Le début est assigné dans \xs_reserved_B et la fin dans \xs_reserved_C
\long\def\xs_StrSplit_ii#1#2{%
	\let\xs_reserved_B\empty\def\xs_reserved_C{#2}\def\xs_reserved_D{#1}\gdef\groupID{}%
	\ifnum#1>0
		\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
		\def\xs_atendofgroup{%
			\edef\__temp{%
				\endgroup
				\noexpand\decimalpart=\number\decimalpart\relax
				\unexpanded{\xs_addtomacro\xs_reserved_B}{{\unexpanded\expandafter{\xs_reserved_B}}}%
				}%
			\__temp
		}%
		\def\xs_atbegingroup{\let\xs_reserved_B\empty}%
		\def\xs_atnextsyntaxunit{%
			\xs_eaddtomacro\xs_reserved_B{\xs_reserved_A}%
			\xs_ifnum{\decimalpart=\xs_reserved_D\relax}
				{\ifx\xs_reserved_C\empty\xs_reserved_E\fi
				\edef\__temp{\def\noexpand\xs_reserved_B{\unexpanded\expandafter{\xs_reserved_B}}\def\noexpand\xs_reserved_C{\unexpanded\expandafter{\xs_reserved_C}}}%
				\expandafter\xs_exitallgroups\__temp
				\xs_gobarg% mange l'appel récursif \xs_read_reserved_C dans \xs_read_reserved_C
				}
				{}%
		}%
		\xs_read_reserved_C
	\fi
}

\def\xs_StrSplit_iii#1#2{\let#1\xs_reserved_B\let#2\xs_reserved_C}

% StrCut[n]{<texte>}{<motif>}\macroA\macroB
% \macroA reçoit ce qui se trouve avant la n ème occurrence <motif> dans <texte>
% \macroB reçoit ce qui est après cette n ème occurrence
\xs_newmacro*3\StrCut{1}{2}{0}{%
	\xs_ifempty{#3}%
		{\gdef\groupID{}\let\xs_reserved_C\empty\let\xs_reserved_E\empty
		}
		{\xs_ifnum{#1<1 }
			{\xs_StrCut_ii{#2}{#3}1}
			{\xs_StrCut_ii{#2}{#3}{#1}}%
		}%
	\xs_StrCut_iii
}

\long\def\xs_StrCut_ii#1#2#3{%
	\let\xs_reserved_C\empty\def\xs_reserved_D{#1}\def\xs_reserved_E{#2}%
	\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
	\def\xs_atoccurfound{%
		\xs_ifnum{\decimalpart=\numexpr(#3)\relax}
			{\edef\__temp{%
				\def\noexpand\xs_reserved_C{\unexpanded\expandafter{\xs_reserved_C}}%
				\def\noexpand\xs_reserved_D{\unexpanded\expandafter{\xs_reserved_D}}%
				\noexpand\decimalpart=\number\decimalpart\relax
				}%
			\expandafter\xs_exitallgroups\__temp
			\xs_gobarg% stoppe la récursivité dans \xs_read_reserved_D
			}
			{\xs_eaddtomacro\xs_reserved_C{\xs_reserved_E}%
			}%
	}%
	\xs_read_reserved_D
	\let\xs_reserved_E\xs_reserved_D
	\xs_exparg{\def\xs_reserved_D}{\xs_reserved_C#2}%
}

\long\def\xs_StrCut_iii#1#2{\let#1\xs_reserved_C\let#2\xs_reserved_E}

% De la chaine #1, renvoie ce qui se trouve entre les positions
%  #2 et #3, unités syntaxiques aux positions compris !
\xs_newmacro\StrMid{}{3}{1}{%
	\begingroup
		\noexploregroups
		\let\xs_reserved_E\relax
		\xs_StrSplit_ii{#3}{#1}%
		\edef\xs_reserved_C{\number\numexpr#2-1}%
		\let\xs_reserved_E\relax
		\xs_exptwoargs\xs_StrSplit_ii\xs_reserved_C\xs_reserved_B
	\expandafter\endgroup
	\expandafter\xs_assign_xstringresult\expandafter{\xs_reserved_C}{#4}%
	\gdef\groupID{}%
}

% supprime #2 unités syntaxiques à gauche dans la chaine #1
\xs_newmacro\StrGobbleLeft{}{2}{1}{%
	\let\xs_reserved_E\relax
	\xs_StrSplit_ii{#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#3}%
}

% extrait de #1 la chaine à gauche de longueur #2
\xs_newmacro\StrLeft{}{2}{1}{%
	\let\xs_reserved_E\relax
	\xs_StrSplit_ii{#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#3}%
}

% supprime #2 unités syntaxiques à droite dans la chaine #1
\xs_newmacro\StrGobbleRight{}{2}{1}{%
	\xs_StrLen{#1}[\xs_reserved_D]%
	\let\xs_reserved_E\relax
	\xs_exparg\xs_StrSplit_ii{\number\numexpr\xs_reserved_D-#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#3}%
}

% renvoie #2 unités syntaxiques à la droite de la chaine #1
\xs_newmacro\StrRight{}{2}{1}{%
	\xs_StrLen{#1}[\xs_reserved_D]%
	\let\xs_reserved_E\relax
	\xs_exparg\xs_StrSplit_ii{\number\numexpr\xs_reserved_D-#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#3}%
}

\xs_newmacro\StrChar{}{2}{1}{%
	\let\xs_reserved_B\empty\def\xs_reserved_C{#1}\def\xs_reserved_D{#2}%
	\ifnum#2>0
		\def\groupID{0}\def\xs_nestlevel{0}\integerpart0 \decimalpart0
		\let\xs_atbegingroup\relax
		\def\xs_atendofgroup{\expandafter\endgroup\expandafter\decimalpart\number\decimalpart\relax}%
		\def\xs_atnextsyntaxunit{%
			\ifnum\decimalpart=\xs_reserved_D% la n ième US est atteinte ?
				\edef\__temp{\def\noexpand\xs_reserved_B{\unexpanded\expandafter{\xs_reserved_A}}}% on capture l'US en cours qui est celle cherchée
				\expandafter\xs_exitallgroups\__temp
				\expandafter\xs_gobarg% stoppe la récursivité dans \xs_read_reserved_C
			\fi
		}%
		\xs_read_reserved_C
	\fi
	\xs_exparg\xs_ifempty{\xs_reserved_B}%
		{\gdef\groupID{}}
		{}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#3}%
}

% Combien de fois compte t-on #2 dans #1 ?
\xs_newmacro\StrCount{}{2}{1}{%
	\def\xs_reserved_D{#1}\def\xs_reserved_E{#2}\let\xs_reserved_C\empty
	\xs_ifempty{#2}%
		{\xs_assign_xstringresult{0}{#3}%
		}
		{\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
		\def\xs_atoccurfound{\let\xs_reserved_C\empty\xs_read_reserved_D}%
		\xs_read_reserved_D
		\xs_exparg\xs_assign_xstringresult{\number\decimalpart}{#3}%
		}%
}

% renvoie la position de l'occurrence #1 de la sous chaine #3 dans la chaine #2
\xs_newmacro\StrPosition{1}{2}{1}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\let\xs_reserved_E\groupID
	\xs_ifx{\xs_reserved_C\xs_reserved_D}
		{\xs_assign_xstringresult{0}{#4}%
		\let\xs_reserved_E\empty
		}
		{\xs_exparg\xs_StrLen{\xs_reserved_C}[\xs_reserved_C]%
		\xs_exparg\xs_assign_xstringresult{\number\numexpr\xs_reserved_C+1}{#4}%
		}%
	\global\let\groupID\xs_reserved_E
}

\def\comparestrict{\def\xs_comparecoeff{1}}
\def\comparenormal{\def\xs_comparecoeff{0}}
\def\savecomparemode{\let\xs_saved_comparecoeff\xs_comparecoeff}
\def\restorecomparemode{\let\xs_comparecoeff\xs_saved_comparecoeff}

% Compare les deux arguments #1 et #2
% Renvoie 0 s'ils sont égaux et renvoie la
% position de la premiere unité syntaxiques différente sinon
\xs_newmacro*2\StrCompare{}{2}{1}{%
	\def\xs_reserved_A{#1}%
	\def\xs_reserved_B{#2}%
	\xs_ifx{\xs_reserved_B\xs_reserved_A}
		{\xs_assign_xstringresult{0}{#3}}
		{\xs_StrCompare_i{#1}{#2}{#3}}%
}

\long\def\xs_StrCompare_i#1#2#3{%
	\def\xs_StrCompare_iii##1{%
		\let\xs_reserved_A\empty
		\xs_exparg\xs_ifempty{\xs_reserved_C}%
			{\edef\xs_reserved_A{*\xs_comparecoeff}}%
			{\xs_exparg\xs_ifempty{\xs_reserved_D}%
				{\edef\xs_reserved_A{*\xs_comparecoeff}}
				{}%
			}%
		\def\xs_next{\xs_exparg\xs_assign_xstringresult{\number\numexpr##1\xs_reserved_A\relax}{#3}}%
	}%
	\def\xs_StrCompare_ii##1{% ##1 est la position
		\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_A
		\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_D}\xs_reserved_B
		\xs_ifx{\xs_reserved_B\xs_reserved_A}
			{\xs_exparg\xs_ifempty{\xs_reserved_A}%
				{\xs_StrCompare_iii{##1}% les 2 unités syntaxiques sont égales, on renvoie la position
				}
				{\def\xs_next{\xs_exparg\xs_StrCompare_ii{\number\numexpr##1+1}}% les 2 unités syntaxiques sont égales et non vides, on recommence
				\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
				\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_D}\xs_reserved_D
				}%
			}% les 2 unités syntaxiques sont différentes : on renvoie la position
			{\xs_StrCompare_iii{##1}%
			}%
		\xs_next
	}%
	\def\xs_reserved_C{#1}\def\xs_reserved_D{#2}%
	\xs_StrCompare_ii1%
}

\xs_newmacro\StrFindGroup{}{2}{1}{%
	\def\xs_reserved_A{#2}\def\xs_reserved_B{0}%
	\xs_ifx{\xs_reserved_A\xs_reserved_B}
		{\xs_assign_xstringresult{{#1}}{#3}}
		{\xs_StrFindGroup_i{#1}{#2}[#3]}%
}

\long\def\xs_StrFindGroup_i#1#2[#3]{%
	\def\xs_StrFindGroup_ii{%
		\xs_exparg\xs_ifempty{\xs_reserved_C}%
			{\xs_assign_xstringresult{}{#3}% s'il ne reste plus rien, on renvoie vide
			}
			{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_D
			\xs_ifx{\bgroup\xs_toks}% si la 1ère unité syntaxique est un groupe explicite
				{\advance\decimalpart1 % on augmente le compteur
				\xs_ifnum{\decimalpart=\xs_reserved_A\relax}% on est au groupe cherché lors de la profondeur courante ?
					{\xs_ifx{\empty\xs_reserved_B}% on est à la profondeur maximale ?
						{\xs_exparg\xs_assign_xstringresult{\xs_reserved_D}{#3}}% on renvoie ce groupe
						{\xs_exparg{\expandafter\xs_StrFindGroup_i\xs_reserved_D}{\xs_reserved_B}[#3]}% on recommence avec ce groupe et les profondeurs de recherche restantes
					}
					{\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
					\xs_StrFindGroup_ii
					}%
				}
				{\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
				\xs_StrFindGroup_ii
				}%
			}%
	}%
	\xs_extractgroupnumber{#2}\xs_reserved_A\xs_reserved_B
	\decimalpart0
	\xs_ifnum{\xs_reserved_A>0 }
		{\def\xs_reserved_C{#1}}
		{\let\xs_reserved_C\empty}%
	\xs_StrFindGroup_ii
}

\def\xs_extractgroupnumber#1#2#3{%
	\def\xs_extractgroupnumber_i##1,##2\_nil{\def#2{##1}\def#3{##2}}%
	\xs_extractgroupnumber_i#1,\_nil
	\ifx\empty#3\else\xs_extractgroupnumber_i#1\_nil\fi
}

\def\expandingroups{\let\xs_expandingroups\exploregroups}

\def\noexpandingroups{\let\xs_expandingroups\noexploregroups}

\def\StrExpand{\xs_testopt{\xs_StrExpand}{1}}
\long\def\xs_StrExpand[#1]#2#3{%
	\begingroup
		\xs_expandingroups
		\xs_ifnum{#1>0 }
			{\integerpart#1 \decimalpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
			\def\xs_atendofgroup{\xs_endgroup_eaddtomacro\xs_reserved_B{\expandafter{\xs_reserved_B}}}%
			\def\xs_atbegingroup{\let\xs_reserved_B\empty}%
			\def\xs_atnextsyntaxunit{\xs_eeaddtomacro\xs_reserved_B{\xs_reserved_A}}%
			\def\xs_reserved_C{#2}%
			\xs_StrExpand_i{#1}% Appel de la macro récursive
			}
			{\def\xs_reserved_B{#2}%
			}
		\expandafter
	\endgroup
	\expandafter\def\expandafter#3\expandafter{\xs_reserved_B}%
	\gdef\groupID{}%
}

\long\def\xs_StrExpand_i#1{%
	\xs_ifnum{#1>0 }
		{\let\xs_reserved_B\empty
		\xs_read_reserved_C
		\let\xs_reserved_C\xs_reserved_B
		\def\xs_reserved_A{\xs_exparg\xs_StrExpand_i{\number\numexpr#1-1}}%
		}
		{\let\xs_reserved_A\relax
		}%
	\xs_reserved_A
}

\def\scancs{\xs_testopt{\xs_scancs}{1}}
\long\def\xs_scancs[#1]#2#3{%
	\xs_StrExpand[#1]{#3}{#2}%
	\edef#2{\detokenize\expandafter{#2}}%
}

\restorexstringcatcode

\setverbdelim{|}%
\fullexpandarg\saveexpandmode
\comparenormal\savecomparemode
\noexploregroups\saveexploremode
\expandingroups

\endinput

                        H I S T O R I Q U E
------------------------------------------------------------------------------
v1.0    4/7/2008 : - Package achevé.
         7/7/2008 : - Package publié sur CTAN.
------------------------------------------------------------------------------
v1.1    15/8/2008
   - Le package ne nécessite plus LaTeX et est désormais utilisable sous
     Plain eTeX.
   - Ajout des macros \IfInteger et \IfDecimal.
     Pour cette dernière, la partie entière et la partie décimale sont
     récupérables dans les compteurs \integerpart et \decimalpart. Ce
     qu'il reste après qu'un caractère non attendu soit rencontré est
     dispo dans \xs_remainafterdecimal
   - Correction d'un bug dans \tokenize :
        suppression de l'expansion avec \normalexpandarg pour éviter le bug
        avec les lettres accentuées dans l'exemple : \tokenize\aa{éù}
   - Amélioration du code de la plupart des macros.
   - écriture d'une routine \xs_newmacro définissant les  macros.
   - Suppression de tous les compteurs grace à \numexpr.
   - Nouvelles fonctionnalités internes dans :
      \IfSubStr
        ajout des chaines se trouvant avant et après l'occurrence testée
        dans les sc \xs_behind_IfSubStr et \xs_before_IfSubStr
      \StrCount
        a) ajout de ce qui se trouve après la dernière occurrence dans la
           sc \xs_StrCount_afterlastocccur
        b) la macro ne dépend plus d'aucune autre
------------------------------------------------------------------------------
v1.2    23/8/2008
   - Amélioration du code de \StrMid \StrGobbleLeft, \StrLeft,
     \StrGobbleRight et \StrRight à l'aide de la nouvelle macro
     \xs_StrSplit_i
   - Nouveau test \IfStrEq qui compare 2 chaines
   - Nouveau test \IfEq qui compare 2 chaines (ou 2 nombres si les 2 chaines
     contiennent un nombre)
   - Correction d'un bug dans \xs_formatnumber. La macro n'envisageait pas le
     cas où son argument était vide ce qui faiasait planter
     \IfDecimal{}{V}{F} et \IfInteger{}{V}{F}
------------------------------------------------------------------------------
v1.3    21/9/2008
  - Amélioration du code, mise en place de récursivités terminales dans
    toutes les macros récursives, simplification de \xs_TestEqual en
    utilisant \ifx
  - Nouvelles macros \IfStrEqCase et \IfEqCase
      Teste si une chaîne est égale à plusieurs chaines données et
      exécute un code spécifique
  - Création de la macro publique \StrSplit
      Coupe la chaine en 2 à une position donnée
  - Nouvelle macro \StrCompare
      Compare 2 chaînes et renvoie la position du 1er caractère différent.
      Renvoie 0 si elles sont égales.
------------------------------------------------------------------------------
v1.3a   29/9/2008
  - Correction d'un bug : \expandafter#1
    dans les macros \IfSubStrBefore et \StrBetween qui buggue si #1 est un
    nombre > 9 !
  - Ré écriture de \xs_returnfirstsyntaxunit et \xs_gobarg qui
    deviennent purement développables.
  - Ré écriture de \StrLen
  - Nouvelle macro interne \xs_cutafteroccur
      Coupe la chaine après la nième occurrence d'une sous chaine.
  - Code amélioré de \StrMid, \StrLeft, \StrGobbleLeft, \StrRight,
    \StrGobbleRight grace à \xs_cutafteroccur
------------------------------------------------------------------------------
v1.4   4/11/2008
  - xstring traite ses arguments par unité syntaxique, et donc toutes les
    macros internes ont été ré-écrites à cette fin.
  - Le manuel a été ré-écrit, rendu plus clair et mieux structuré.
  - Nouvelle fonctionnalité : \expandarg
      le 1er lexème de chaque argument est 1-développé avant que la
      macro ne soit appelée. Si un argument comporte plus qu'1 lexème,
      il faut passer par \scancs*[1] pour 1-développer toutes les unités
      syntaxiques.
  - Correction de 2 erreurs dans le manuel anglais :  0 est la valeur par
    défaut dans \StrSubstitute et \StrDel
  - Cohérence dans les nom des séquences de contrôles temporaires qui
    sont désormais : \xs_reserved_A à \xs_reserved_E
------------------------------------------------------------------------------
v1.4a  12/11/2008
  - Correction d'un bug dans \xs_StrSplit dans le cas où l'argument
     numérique est <1 : la 1ere coupure doit être vide et le seconde doit
     être égale à l'argument.
------------------------------------------------------------------------------
v1.4b  16/11/2008
  - Correction de 2 bugs dans \xs_returnfirstsyntaxunit
------------------------------------------------------------------------------
v1.5   31/12/2008
  - Nouvelles fonctionnalités dans la recherche de groupes par un
    identificateur caractérisant leur imbrication. Implémentation de :
      1) \StrFindGroup
      2) \groupID
  - Ajout des nouvelles macros génériques \xs_read_reserved_C et
    \xs_read_reserved_D
  - Correction d'un bug dans \StrSplit : \StrSplit{{a}bc}{1}[\truc] faisait
    que \truc contenait «a{a}».
  - Correction d'un bug dans \xs_newmacro : l'argument optionnel était
    détokénisé à tort dans les macros étoilées.
  - Dans \xs_newmacro, on doit choisir le numéro du dernier argument devant
    être détokénisé dans le cas d'une macro étoilée (sachant que
     l'argument optionnel ne l'est jamais)
------------------------------------------------------------------------------
v1.5a  09/2/2009
  - Nouvelle macro \StrExpand, sensible au mode d'exploration. La macro est
    indépendante du mode d'exploration et dispose de ses propres commandes
    d'exploration : \expandingroups et \noexpandingroups
  - Ré-écriture de \scancs, qui devient triviale puisque dépendant de
    \StrExpand. Il n'y a plus de version étoilée et désormais, \scancs
    est sensible au mode d'exploration.
  - Correction d'un bug dans \IfInteger : \IfInteger{2.0}{V}{F} affichait F
  - Correction de bugs : mettre \let\xs_reserved_E\relax avant d'appeler
    \xs_StrSplit_i
  - Suppression des messages d'erreur, de warning et d'info. xstring devient
    donc silencieux ;)
  - Passage de 3 à 2 compteurs
  - Le manuel est désormais plus coloré, en espérant qu'il sera un peu
    plus agréable à lire !
------------------------------------------------------------------------------
v1.5b  13/3/2009
  - Modification d'un grand nombre de macros de telle sorte que vraiment
    n'importe quel code peut désormais être placé dans les arguments des
    macros (comme par exemple des \if, \ifx ou autre, même sans leur \fi, ce
    qui n'était pas possible jusqu'alors)
------------------------------------------------------------------------------
v1.5c  05/6/2009
  - Correction d'un bug dans \IfBeginWith : il faut appeler
    \xs_returnfirstsyntaxunit pour l'argument #2 puis pour l'argument #1 et
    non pas l'inverse pour que \xs_toks reflète ce qui se trouve dans #1
  - Correction d'un bug dans \xs_returnfirstsyntaxunit au cas où #1 commence
    par un espace : mettre \xs_toks à 0
  - Correction d'un bug dans \xs_returnfirstsyntaxunit :
    \xs_returnfirstsyntaxunit{{}}\truc
    faisait que \truc se développait en un espace.
  - Correction d'un bug dans \xs_removefirstsyntaxunit où le cas
    \xs_removefirstsyntaxunit{ {b}}\truc
    donnait \truc se développant en «b» au lieu de «{b}».
------------------------------------------------------------------------------
v1.5d  28/3/2010
  - Correction d'un bug dans \IfInteger : \afterinteger ne donnait pas le
    bon résultat. Par exemple avec 1.23 il renvoyait {} au lieu de {.23}
  - \xs_formatnumber ne detokenize plus ses arguments (que m'est-il passé
    par la tête pour que je code un truc comme ca ?), et donc
    \afterinteger et \xs_afterdecimal ont des tokens ayant le bon
    catcode
------------------------------------------------------------------------------
v1.6  24/10/2012
  - Correction d'un bug dans \xs_cutafteroccur au cas où #3<1
  - \IfDecimal ne \detokenize plus l'argument.
  - Nouvelle version de \tokenize qui enlevait les accolades si son argument
    était entre accolades
  - Nouvelle macro \StrCut
  - \xs_cutafteroccur_i ne produit plus d'espace indésirable si #3 était
    évalué par \numexpr
------------------------------------------------------------------------------
v1.7  13/1/2013
  - Correction d'un manque de rigueur dans les assignations concernant
    \groupID : elles sont toutes globales désormais
  - Les macros de xstring sont \long
------------------------------------------------------------------------------
v1.7a 28/2/2013
  - Correction d'un espace parasite dans \xs_removefirstsyntaxunit
------------------------------------------------------------------------------
v1.7b 29/7/2013
  - La date contenue dans \xstringdate est désormais conforme
------------------------------------------------------------------------------
v1.7c 13/10/2013
  - les macros impliquées dans \IfStrCase et \IfStrEqCase sont désormais \long
------------------------------------------------------------------------------
v1.8  07/12/2018
  - affectations globales supprimées (sauf pour \groupID) afin de ne pas
    surcharger la pile de sauvegarde
  - nettoyage du code, corrections de lourdeurs et maladresses
------------------------------------------------------------------------------
v1.81 09/12/2018
  - bug dans \IfInteger et \IfDecimal, la macro \xs_afterdecimal est indéfinie
    et doit être remplacée par \afterdecimal
------------------------------------------------------------------------------
v1.82 01/02/2019
  - \xs_testopt n'est pas longue et provoque un bug dans \xs_IfStrCase et
    \xs_IfStrCase lorsque #1 contient \par : \xs_testopt reste courte et
    \xs_IfStringCase a été modifiée pour que cela fonctionne.
    ------------------------------------------------------------------------------
v1.83 06/02/2019
      - mauvaise approche et mauvais fix dans la v1.82 : \xs_testopt devient
        longue, pas le choix (et donc aussi \xs_ifnxttok)
